Variable Selection with Rigorous Uncertainty Quantification using Deep Bayesian Neural Networks: Posterior Concentration and Bernstein-von Mises Phenomenon

This work develops rigorous theoretical basis for the fact that deep Bayesian neural network (BNN) is an effective tool for high-dimensional variable selection with rigorous uncertainty quantification. We develop new Bayesian non-parametric theorems to show that a properly configured deep BNN (1) learns the variable importance effectively in high dimensions, and its learning rate can sometimes "break" the curse of dimensionality. (2) BNN's uncertainty quantification for variable importance is rigorous, in the sense that its 95% credible intervals for variable importance indeed covers the truth 95% of the time (i.e., the Bernstein-von Mises (BvM) phenomenon). The theoretical results suggest a simple variable selection algorithm based on the BNN's credible intervals. Extensive simulation confirms the theoretical findings and shows that the proposed algorithm outperforms existing classic and neural-network-based variable selection methods, particularly in high dimensions.

==> preamble/author_article.tex <==
%% Here are the title, author names and addresses
\title{Constrained Gaussian Process for Regression, Classification and Distribution Estimation}

\author{Jeremiah Z. Liu\thanks{zhl112@mail.harvard.edu.}}
\affil{Department of Biostatistics, Harvard University, Boston, MA, USA.}
\date{}


==> preamble/author_biometrika.tex <==
%% The left and right page headers are defined here:
\markboth{}{}

%% Here are the title, author names and addresses
\title{
Quantifying Uncertainty in Feature Selection \\ 
with Bayesian Deep  Networks
}

\author{Jeremiah Z. Liu* \thanks{* Work in progress.}}
\affil{Department of Biostatistics, Harvard University,\\ Boston, MA, USA \email{zhl112@mail.harvard.edu.}}


==> preamble/author_jmlr.tex <==
% Short headings should be running head and authors last names
\ShortHeadings{Feature Selection with Rigorous Uncertainty Quantification using Deep BNN}{Liu}
\firstpageno{1}

\begin{document}

\title{Simple Feature Selection with Rigorous Uncertainty Quantification using Bayesian Deep Neural Networks:\\
Sparsistency and Bernstein-von Mises Phenomenon}

\author{\name Jeremiah Zhe Liu \email zhl112@mail.harvard.edu \\
       \addr Department of Biostatistics\\
       Harvard University\\
       Boston, MA 02115, USA
%       \AND
%       \name Michael I.\ Jordan \email jordan@cs.berkeley.edu \\
%       \addr Division of Computer Science and Department of Statistics\\
%       University of California\\
%       Berkeley, CA 94720-1776, USA
       }

\editor{}


==> preamble/definition.tex <==
% author comment
\newcommand{\jzl}[1]{{\color{brown} (\textbf{jzl:} #1)}}
\newcommand{\bac}[1]{{\color{red} (\textbf{bac:} #1)}}
\newcommand{\ram}[1]{{\color{blue} (\textbf{ram:} #1)}}

% symbols
\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}

% inner product
\newcommand\inner[2]{\langle #1, #2 \rangle}

% theorem
\newtheorem{theorem_app}{Theorem}[section]
\newtheorem{assumption}{Assumption}

% parfor blocks
\algblock{ParFor}{EndParFor}
% customising the new block
\algnewcommand\algorithmicparfor{\textbf{parfor}}
\algnewcommand\algorithmicpardo{\textbf{do}}
\algnewcommand\algorithmicendparfor{\textbf{end\ parfor}}
\algrenewtext{ParFor}[1]{\algorithmicparfor\ #1\ \algorithmicpardo}
\algrenewtext{EndParFor}{\algorithmicendparfor}

% set equation space
\setlength{\abovedisplayskip}{0pt}%
\setlength{\belowdisplayskip}{0pt}%
\setlength{\abovedisplayshortskip}{0pt}%
\setlength{\belowdisplayshortskip}{0pt}%
\setlength{\jot}{0pt}% Inter-equation spacing

==> preamble/packages_article.tex <==
\makeatletter
\providecommand{\@LN}[2]{}
\makeatother

\usepackage[margin=1in]{geometry}
\usepackage{times}
\usepackage{graphicx,psfrag,epsf}
\usepackage{enumerate}
\usepackage{natbib}
\usepackage{url} % not crucial - just used below for the URL 
\usepackage{setspace}
\setstretch{1.8}

%\pdfminorversion=4
% NOTE: To produce blinded version, replace "0" with "1" below.
\newcommand{\blind}{0}

\newlength\tindent
\setlength{\tindent}{\parindent}
\setlength{\parindent}{0pt}
\renewcommand{\indent}{\hspace*{\tindent}}

% DON'T change margins - should be 1 inch all around.
% \addtolength{\oddsidemargin}{-.5in}%
% \addtolength{\evensidemargin}{-.5in}%
% \addtolength{\textwidth}{1in}%
% \addtolength{\textheight}{-.3in}%
% \addtolength{\topmargin}{-.8in}%

%  If your system does not have the AMS fonts version 2.0 installed, then
%  remove the useAMS option.
%
%  useAMS allows you to obtain upright Greek characters.
%  e.g. \umu, \upi etc.  See the section on "Upright Greek characters" in
%  this guide for further information.
%
%  If you are using AMS 2.0 fonts, bold math letters/symbols are available
%  at a larger range of sizes for NFSS release 1 and 2 (using \boldmath or
%  preferably \bmath).
% 
%  Other options are described in the user guide. Here are a few:
% 
%  -  If you use Patrick Daly's natbib  to cross-reference your 
%     bibliography entries, use the usenatbib option
%
%  -  If you use \includegraphics (graphicx package) for importing graphics
%     into your figures, use the usegraphicx option
% 
%  If you wish to typeset the paper in Times font (if you do not have the
%  PostScript Type 1 Computer Modern fonts you will need to do this to get
%  smoother fonts in a PDF file) then uncomment the next line
%  \usepackage{Times}

% to compile a camera-ready version, add the [final] option, e.g.:
% \usepackage[final]{nips_2017}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{comment}      % comment
\usepackage{multirow}

%
\usepackage{graphicx}
\usepackage{subcaption}


% 
\usepackage{amsmath}
\usepackage{amssymb, mathtools}
\usepackage{amsfonts}
\usepackage{mathptmx}
\usepackage{amsthm}

%
\usepackage{algorithm}
\usepackage{algpseudocode}

% use glossary
\usepackage
[acronym,nowarn,section,nonumberlist]{glossaries}
\glsdisablehyper{}

%
\usepackage{authblk}

%
\usepackage{color} % pre-req for below macros
\usepackage{xcolor}
\usepackage{"./macro/GrandMacros"}
\usepackage{"./macro/Macro_BIO235"}

% theorem
\newtheoremstyle{break}
  {\topsep}{\topsep}%
  {\itshape}{}%
  {\bfseries}{}%
  {\newline}{}%
  
\theoremstyle{break}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}


==> preamble/packages_biometrika.tex <==
\usepackage{amsmath}

%% Please use the following statements for
%% managing the text and math fonts for your papers:
\usepackage{times}
%\usepackage[cmbold]{mathtime}
\usepackage{bm}
\usepackage{natbib}

\usepackage[plain,noend]{algorithm2e}

\makeatletter
\renewcommand{\algocf@captiontext}[2]{#1\algocf@typo. \AlCapFnt{}#2} % text of caption
\renewcommand{\AlTitleFnt}[1]{#1\unskip}% default definition
\def\@algocf@capt@plain{top}
\renewcommand{\algocf@makecaption}[2]{%
  \addtolength{\hsize}{\algomargin}%
  \sbox\@tempboxa{\algocf@captiontext{#1}{#2}}%
  \ifdim\wd\@tempboxa >\hsize%     % if caption is longer than a line
    \hskip .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}% then caption is not centered
  \else%
    \global\@minipagefalse%
    \hbox to\hsize{\box\@tempboxa}% else caption is centered
  \fi%
  \addtolength{\hsize}{-\algomargin}%
}
\makeatother

%%% User-defined macros should be placed here, but keep them to a minimum.
%\def\Bka{{\it Biometrika}}
%\def\AIC{\textsc{aic}}
%\def\T{{ \mathrm{\scriptscriptstyle T} }}
%\def\v{{\varepsilon}}

\addtolength\topmargin{35pt}
\DeclareMathOperator{\Thetabb}{\mathcal{C}}


%\usepackage{times}
\usepackage{graphicx,psfrag,epsf}
\usepackage{enumerate}
\usepackage{natbib}
%\usepackage{url} % not crucial - just used below for the URL 
%\usepackage{setspace}
%\setstretch{1.5}

%
%%\pdfminorversion=4
%% NOTE: To produce blinded version, replace "0" with "1" below.
%\newcommand{\blind}{1}
%
%\newlength\tindent
%\setlength{\tindent}{\parindent}
%\setlength{\parindent}{0pt}
%\renewcommand{\indent}{\hspace*{\tindent}}
%
%% DON'T change margins - should be 1 inch all around.
%%\addtolength{\oddsidemargin}{-.5in}%
%%\addtolength{\evensidemargin}{-.5in}%
%%\addtolength{\textwidth}{1in}%
%%\addtolength{\textheight}{-.3in}%
%%\addtolength{\topmargin}{-.8in}%
%\usepackage[margin=1in]{geometry}
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{comment}      % comment
%\usepackage{multirow}
%
%%
%\usepackage{subcaption}
\usepackage[caption=false]{subfig}
%
%
% 
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{mathptmx}
%
%%
%\DeclarePairedDelimiter{\inner}{\langle}{\rangle}
%\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
%
%%
%\usepackage{algorithm}
%\usepackage{algpseudocode}
%
%% 
%\usepackage{tikz}
%\usetikzlibrary{bayesnet, positioning,shapes.geometric, arrows, fit,calc}
%\tikzstyle{block} = [draw, rectangle, fill=orange!50, text width=8em, text centered, minimum height=15mm, node distance=10em]
%\tikzstyle{container} = [draw, rectangle, dashed, inner sep=0.7em]
%\tikzstyle{arrow} = [thick,->,>=stealth]
%
%%
%\let\proof\relax
%\let\endproof\relax
%\usepackage{amsthm}

%\newtheorem{corollary}{Corollary}[theorem]
%\newtheorem*{lemma}{Definition}

% use glossary
\usepackage
[acronym,nowarn,section,nonumberlist]{glossaries}
\glsdisablehyper{}

% Definitions of handy macros can go here
% macros from Bob Gray

\usepackage{color} % pre-req for below macros
\usepackage{xcolor}
\usepackage{"./macro/GrandMacros"}
\usepackage{"./macro/Macro_BIO235"}

\usepackage{tocstyle}


==> preamble/packages_jmlr.tex <==
% Any additional packages needed should be included after jmlr2e.
% Note that jmlr2e.sty includes epsfig, amssymb, natbib and graphicx,
% and defines many common macros, such as 'proof' and 'example'.
%
% It also sets the bibliographystyle to plainnat; for more information on
% natbib citation styles, see the natbib documentation, a copy of which
% is archived at http://www.jmlr.org/format/natbib.pdf

\usepackage[abbrvbib]{jmlr2e}

% Definitions of handy macros can go here

\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}

% Heading arguments are {volume}{year}{pages}{date submitted}{date published}{paper id}{author-full-names}

%\jmlrheading{1}{2000}{1-48}{4/00}{10/00}{liu19a}{Jeremiah Zhe Liu}


% other packages
\usepackage{amsmath}

%% Please use the following statements for
%% managing the text and math fonts for your papers:
\usepackage{times}
%\usepackage[cmbold]{mathtime}
\usepackage{bm}
\usepackage{natbib}

\usepackage[ruled,vlined,linesnumbered,noresetcount]{algorithm2e}
\usepackage{algcompatible}
\usepackage{algpseudocode}
%\usepackage[plain,noend]{algorithm2e}

\makeatletter
\renewcommand{\algocf@captiontext}[2]{#1\algocf@typo. \AlCapFnt{}#2} % text of caption
\renewcommand{\AlTitleFnt}[1]{#1\unskip}% default definition
\def\@algocf@capt@plain{top}
\renewcommand{\algocf@makecaption}[2]{%
  \addtolength{\hsize}{\algomargin}%
  \sbox\@tempboxa{\algocf@captiontext{#1}{#2}}%
  \ifdim\wd\@tempboxa >\hsize%     % if caption is longer than a line
    \hskip .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}% then caption is not centered
  \else%
    \global\@minipagefalse%
    \hbox to\hsize{\box\@tempboxa}% else caption is centered
  \fi%
  \addtolength{\hsize}{-\algomargin}%
}
\makeatother

%%% User-defined macros should be placed here, but keep them to a minimum.
%\def\Bka{{\it Biometrika}}
%\def\AIC{\textsc{aic}}
%\def\T{{ \mathrm{\scriptscriptstyle T} }}
%\def\v{{\varepsilon}}

\addtolength\topmargin{35pt}
\DeclareMathOperator{\Thetabb}{\mathcal{C}}


%\usepackage{times}
\usepackage{graphicx,psfrag,epsf}
\usepackage{enumerate}
\usepackage{natbib}
%\usepackage{url} % not crucial - just used below for the URL 
%\usepackage{setspace}
%\setstretch{1.5}

\usepackage{comment}

%
%%\pdfminorversion=4
%% NOTE: To produce blinded version, replace "0" with "1" below.
%\newcommand{\blind}{1}
%
%\newlength\tindent
%\setlength{\tindent}{\parindent}
%\setlength{\parindent}{0pt}
%\renewcommand{\indent}{\hspace*{\tindent}}
%
%% DON'T change margins - should be 1 inch all around.
%%\addtolength{\oddsidemargin}{-.5in}%
%%\addtolength{\evensidemargin}{-.5in}%
%%\addtolength{\textwidth}{1in}%
%%\addtolength{\textheight}{-.3in}%
%%\addtolength{\topmargin}{-.8in}%
%\usepackage[margin=1in]{geometry}
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{comment}      % comment
%\usepackage{multirow}
%
%%
%\usepackage{subcaption}
\usepackage[caption=false]{subfig}
%
%
% 
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{mathptmx}
%
%%
%\DeclarePairedDelimiter{\inner}{\langle}{\rangle}
%\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
%
%%
%\usepackage{algorithm}
%\usepackage{algpseudocode}
%
%% 
%\usepackage{tikz}
%\usetikzlibrary{bayesnet, positioning,shapes.geometric, arrows, fit,calc}
%\tikzstyle{block} = [draw, rectangle, fill=orange!50, text width=8em, text centered, minimum height=15mm, node distance=10em]
%\tikzstyle{container} = [draw, rectangle, dashed, inner sep=0.7em]
%\tikzstyle{arrow} = [thick,->,>=stealth]
%
%%
%\let\proof\relax
%\let\endproof\relax
%\usepackage{amsthm}

%\newtheorem{corollary}{Corollary}[theorem]
%\newtheorem*{lemma}{Definition}

% use glossary
\usepackage
[acronym,nowarn,section,nonumberlist]{glossaries}
\glsdisablehyper{}

% multirow table
\usepackage{multirow}
\usepackage{adjustbox}

% Definitions of handy macros can go here
% macros from Bob Gray

\usepackage{color} % pre-req for below macros
\usepackage{xcolor}
\usepackage{"./macro/GrandMacros"}
\usepackage{"./macro/Macro_BIO235"}

\usepackage{tocstyle}

% refering external packages
\usepackage{xr}


==> sections/algorithm.tex <==
Theorem \ref{thm:bvm} suggests a simple variable selection algorithm for deep \gls{ReLU} networks that incorporates model uncertainty and naturally handles the multiple comparison problem. That is, to obtain a variable selection decision with its \gls{FDR} controlled at $\alpha$, we can first compute the $(1-\alpha)$-level simutaneous credible intervals $\{\hat{B}_p\}_{p=1}^P$ for the joint posterior $\Pi\big(\{\psi_p^c(f)\}_{p=1}^P\big)$ \citep{olea_simultaneous_2019}, and then select variable by examining whether each $\hat{B}_p$ contains zero (i.e. $\bbI(0 \not\in \hat{B}_p)$) (Algorithm \ref{alg:var_select}). 

\begin{algorithm}[H]
\SetAlgoLined
\KwIn{$M$ samples of posterior samples $\{\bS_m\}_{m=1}^M$.}
\KwOut{index set of selected variables $\hat{A}_{n}$.}
Initialize $\hat{A}_n=\emptyset$\;
$\{\psi^c_m\}_{m=1}^M = \mbox{compute$\_$variable$\_$importance}(\{\bS_m\}_{m=1}^M)$ \;
$\{\hat{B}_p\}_{p=1}^P=\mbox{compute$\_$simutaneous$\_$interval}(\{\psi_m\}_{m=1}^M)$\;
\For{$p = 1, \dots, P$}{
\If{$0 \not\in \hat{B}_p$}{
$\hat{A}_n = \mbox{insert}(\hat{A}_{n}, p)$\;
}
}
\caption{Variable Selection with Bayesian \gls{ReLU} Network}
\label{alg:var_select}
\end{algorithm}

In the above algorithm, the validity of the decision rule $\bbI(0 \not\in \hat{B}_p)$ is justified by the multivariate  \gls{BvM} theorem (Theorem \ref{thm:bvm_mvn}). Specifically, since the posterior credible set $\hat{B}=\{\hat{B}_p\}_{p=1}^P$ is the $(1-\alpha)$-level simutaneous confidence interval for the true variable importance $\psi(f_0)=\{\psi_p(f_0)\}_{p=1}^P$, $\hat{B}$ is expected to cover $\psi(f_0)$ for $(1-\alpha)\%$ of the time under the data-generation mechanism, thereby serving as a valid criteria for variable selection that offers precise control over its overall \gls{FDR}. 

%Furthermore, since $\hat{B}$ is computed with respect to the joint posterior $\Pi_n(\hat{\psi}(f))$, variable selection with $\hat{B}$ implicitly accounts for the intricate dependency  between the statistical conclusion for different candidate variables $\{x_p\}_{p=1}^P$, thereby naturally handles the multiple comparison problem that is common for high-dimensional variable selection procedures \citep{dehmer_computational_2015}.

%\subsection{Theoretical Guarantee}

The posterior consistency result in Theorem \ref{thm:post_convergence} endow the algorithm further important properties. Specifically, due to the consistency in estimating $\hat{\Psi}_p(f_0)$, the index set of variables selected by Algorithm \ref{alg:var_select} (denoted as $\hat{A}_n$) is guaranteed to recover the set of the truely informative variables for $f_0$ (denoted as $A_0$) with probability 1, an important property for variable selection known as \textit{sparsistency} \citep{ravikumar_sparse_2007}. Furthermore, the covergence speed for $\hat{A}_n \rightarrow A_0$ under Algorithm \ref{alg:var_select} is sufficiently fast, due to the fast convergence of \gls{ReLU} networks in learning variable importance in high-dimensional problems.

\begin{theorem}[Sparsistency]
For $f \in \Fsc(L, K, S, B)$, assuming the posterior distribution $\Pi_n(f)$ contracts around $f_0$ with rate $\epsilon_n$. Given $\{\bx_i, y_i\}_{i=1}^n$, denote $\hat{A}_n$ the index set selected by Algorithm \ref{alg:var_select}, and denote $A_0$ the ``true" index set for $f_0$ (i.e. the set of $p$'s for which $\Psi_p(f_0)=||\deriv{x_p}f_0||^2_2 \neq 0$), then we have for $n \rightarrow \infty$:
\begin{align*}
E_0\Pi \Big(\hat{A}_n = A_0 \big| \{\bx_i, y_i\}_{i=1}^n \Big) \rightarrow 0
\end{align*}
\label{thm:sparsistency}
\end{theorem}
\begin{proof}
See Section \ref{sec:sparsistency_proof}
\end{proof}

==> sections/background_bnn.tex <==
The Bayesian approach to neural network learning specifies a prior distribution $\Pi(f)$ that assigns probability to every candidate $f \in \Fsc(L, K, S, B)$ in the model space. For a neural network model $f(.)=\beta^\top\phi_{\Wsc}(.)$, the prior distribution $\Pi(f)$ is commonly specified through its model weights $\{\beta, \Wsc\}$, i.e., by specifying a hierarchically distribution $\Pi(f, \beta, \Wsc)$:
\begin{align}
\Pi(f, \beta, \Wsc) = \Pi(f|\beta, \Wsc)\Pi(\beta)\Pi(\Wsc),
\label{eq:bnn_prior_pre}
\end{align}
where $\Pi(f|\beta, \Wsc)$ is the Dirac measure $\bbI(f=\beta\phi_{\Wsc})$. $\Pi(\beta)$, $\Pi(\Wsc)$ are the prior distributions for the output and hidden weights of the neural network model.

It is well-known that for some common choices of $\Pi(\beta)$, $\Pi(f)$ corresponds to a (conditional) \glsfirst{GP} \citep{neal_bayesian_1996}. Specifically, by placing \gls{iid} Gaussian prior $N(0, \frac{1}{K})$ on $\beta$ and $N(0, \sigma^2_{b_0})$ on $b_0$, the neural network model $f(.)=\phi_{\Wsc}(.)^\top\beta$ is equal in distribution to Gaussian process with kernel function $k_\Wsc(\bx, \bx')=\frac{1}{K}\phi_{\Wsc}(\bx)^\top\phi_{\Wsc}(\bx') + \sigma_{b_0}^2$, i.e., $\Pi(f|\Wsc) = GP(f|0, k_\Wsc)$. 
\begin{comment}
Given data $\{\bx_i, y_i\}_{i=1}^n$, the kernel matrix is evaluated as $\bK = \frac{1}{K}\bPhi\bPhi^\top$ for $\bPhi_{n \times K}=\bX(\prod_{l=1}^L \bW_l\bS_l)$ (see Section \ref{sec:relu_intro}).
\end{comment} 

As a result, under the conditional \gls{GP} representation, the prior distribution for $f$ can be written as:
\begin{align}
\Pi(f, \Wsc) = \Pi(f|\Wsc)\Pi(\Wsc) = GP(f|0, k_\Wsc)\Pi(\Wsc),
\label{eq:bnn_prior}
\end{align}
where the common choices for $\Pi(\Wsc)$ include Gaussian \citep{neal_bayesian_1996}, Laplace \citep{williams_bayesian_1995}, Spike and Slab \citep{rockova_posterior_2018}, and Horseshoe \citep{ghosh_model_2017, louizos_learning_2018}. 

The conditional GP representation in (\ref{eq:bnn_prior}) is important for analyzing the asymptotic behavior of the Bayesian neural network. It suggests that, if the behavior of the conditional posterior $\Pi_n(f|\Wsc)$ does not change drastically under $\Pi_n(\Wsc)$, then the asymptotic behavior of $\Pi_n(f, \Wsc)$ is analogous to that of a Gaussian process, whose theoretical properties are well-understood in the literature \citep{van_der_vaart_rates_2008, castillo_nonparametric_2013}. In Section \ref{sec:thm_bvm}, we take advantage of this representation to show an \gls{BvM} phenomenon (i.e. asymptotic normality) for the posterior distribution of variable importance for a wide range of choices for $\Pi(\Wsc)$.

\begin{comment}
As an aside, when $K \rightarrow \infty$ (i.e. a neural network with infinite width), the central limit theorem implies that  $\Pi(f, \Wsc)$ in fact converge to a exact \gls{GP} with kernel function $k_\Wsc(\bx, \bx')=E_{\Pi(\Wsc)}(\phi_{\Wsc}(\bx)^\top\phi_{\Wsc}(\bx'))$, which gives arise to the well-known arc-cosine kernel and its deep extensions \citep{cho_kernel_2009, lee_deep_2018}. However, this turns $f$ into a purely nonparametric model, we don't pursue this direction in the current work.
\end{comment}


\subsubsection*{Posterior Consistency and Concentration Rates}

The quality of a Bayesian learning procedure is commonly measured by the learning rate of its posterior distribution, i.e., the speed at which the posterior distribution $\Pi_n$ shrinks around the truth as $n \rightarrow \infty$. Such speed is usually assessed by the radius of a small ball surrounding $f_0$ that contains the majority of the posterior probability mass, i.e., a set $A_n = \{f | ||f - f_0||_n \leq M\epsilon_n\}$ such that $\Pi_n(A_n)\rightarrow 1$. Here, the \textit{concenration rate} $\epsilon_n$ describes how fast this small ball concentrates toward $f_0$ as the sample size increases. Clearly, an efficient Bayesian learning procedure that has good finite-sample performance is expected to have an $\epsilon_n$ that converges quickly to zero. 

We state the notion of posterior concentration formally as below \citep{ghosal_convergence_2007}:

\begin{definition}[Posterior Concentration]
For $f^* \in \Fsc^*$ where $d = o(1)$, let $\Fsc(L, K, S, B)$ denote a class of \gls{ReLU} network with depth $L$, width $W$,  sparsity bound $S$ and norm bound $B$. Also denote $f_0$ the \gls{KL}-projection of $f^*$ to $\Fsc(L, K, S, B)$, and $E_0$ the expectation with respect to $P_0$. Then we say the posterior distribution $f$ concentrates around $f_0$ at the rate $\epsilon_n$ in $\Pbb^{n}_0$ probability if, for any $M_n \rightarrow \infty$, there exists an $\epsilon_n \rightarrow 0$ such that $n \epsilon_n^2 \rightarrow \infty$ and:
\begin{align}
E_0\Pi(f: ||f - f_0||^2_n > M_n \epsilon_n | \{y_i, \bx_i\}_{i=1}^n ) \rightarrow 0
\label{eq:f_post_converg}
\end{align}
\label{def:post_conv}
\end{definition}
%Notice that the above notion of posterior concentration concerns not about the the true target function $f^*$ itself, but rather the projection of $f^*$ onto the model space $\Fsc$. This is because without explicit assumptions about the property of $f^*$ (e.g. smoothness), there is no guarantee that $\Fsc$ can well approximate $f^*$ even when the same size increases to infinity (i.e. non-vanishing asymptotic bias). However, under mild assumptions, it can be shown that the posterior distribution will converge to a point in $\Fsc$ that is closest to $f^*$ in the \gls{KL} sense, i.e. $f_0$ \citep{ramamoorthi_posterior_2015}.
To ensure the full generality of our theoretical results, in this work we do not assume an specific expression for $\epsilon_n$ (except that it is upper bounded by the optimal parametric rate  $O(n^{-1/2})$), requiring only that such rate $\epsilon_n \rightarrow 0$ exists and is attained by the \gls{ReLU} network configured by the user. In practice, the exact value of the concenration rate $\epsilon_n$ depends on the property of the learning problem. Specifically, $\epsilon_n$ depends on the dimension of the input feature $P$, and the geometry of the ``true" function space $f^* \in \Fsc^*$. For example, under the typical nonparametric assumption that $\Fsc^* = \Hsc^\beta$ is the space of $\beta$-H\"{o}lder smooth (i.e. $\beta$-times differentiable) functions, the concentration rate $\epsilon_n$ is found to be close to minimax optimal up to a logarithm factor, i.e., $\epsilon_n = O\big( n^{-2\beta/(2\beta + P)} * (log \, n)^{\gamma} \big)$ for some $\gamma > 1$ \citep{rockova_posterior_2018}. However, recent advances in frequentist learning theory shows that a deep \gls{ReLU} network model can surpass the optimal nonparametric rate by adapting to the structure of $f^*$ \citep{bach_breaking_2014, suzuki_adaptivity_2018} and to the intrinsic dimension of the input feature space \citep{nakada_adaptive_2019}, suggesting that the Bayesian concetration rate $\epsilon_n$ can achieve similar adaptivity as well. In particular, if $\Fsc^*=\Fsc(L, K, S, B)$ (i.e. the target function lies in the approximation  space of the neural networks), it can be shown that even under the standard \gls{iid} Gaussian prior, $\epsilon_n$ can achieve a fast polynomial rate of $O(n^{-\frac{1}{2}})$ (up to a logarithm factor). %This result appear to be new to the literature, and we give a complete statement and full proof in Proposition \ref{thm:f_post_converg}. 

%If one is willing to make explicit assumptions about $\Fsc^*$ (e.g. $f^* \in \Fsc^*$ a H\"{o}lder space with certain smoothness level $\beta$), then it is possible to discuss posterior concentration toward the the target function $f^*$ itself, e.g. by investigating the convergence behavior of $\Pi_n(f: ||f - f^*||_n > M_n \epsilon_n)$. To do so, one need to characterize the convergence behavior of the approximation error $\inf_{f_0 \in \Fsc} |f_0 - f^*|$ by leveraging function approximation theory for \gls{ReLU} networks, and then incorporate such approximation error into the rate of concetration $\epsilon_n$ (see, e.g. \cite{schmidt-hieber_nonparametric_2017}). For example, if assuming $f^* \in \Hsc_d^\beta$, the concentration rate $\epsilon_n$ is found to be close to minimax optimal $\epsilon_n = O\Big( n^{-\frac{2\beta}{2\beta + d}} * (log \, n)^{\gamma} \Big)$ for some $\gamma > 1$ \citep{rockova_posterior_2018}.


==> sections/background_nn.tex <==
\subsection{Deep \gls{ReLU} Neural Network}
\label{sec:relu_intro}

Denote the \gls{ReLU} activation function $\sigma: \real^K \rightarrow \real^K$ as the element-wise ramp function $\sigma(\bh) = [max(0, h_1), \dots, max(0, h_K)]$ for a vector $\bh = [h_1, \dots, h_K]$. The class of deep \gls{ReLU} neural networks with depth $L$ and width $K$ can be written as
\begin{align*}
f(\bx) 
= 
b_0 + \beta^\top \Big[ \circ_{l=1}^L (\sigma \Wsc_l) \circ x \Big] = 
b_0 + \beta^\top \Big[ \sigma \Wsc_L \Big(\sigma \Wsc_{L-1} \dots \big( \sigma \Wsc_2 (\sigma \Wsc_1 \bx) \big)\Big)\Big],
\end{align*}
where $b_0 \in \real$ and $\beta \in \real^K$ are the bias and the  weights for the output layer, $\Wsc_l \in \real^{K \times K}$ for $l \geq 2$ are weights for the hidden layers, and $\Wsc_1 \in \real^{K \times P}$ is the weight matrix for the input layer. We denote the collection of hidden layers as $\Wsc = \{\Wsc_l\}_{l=1}^L$. Following existing approaches in deep learning theory \citep{schmidt-hieber_nonparametric_2017, suzuki_adaptivity_2018}, we assume the hidden weights $\Wsc$ satisfy the sparsity constraint $\Csc^S_0$ and norm constraint $\Csc^B_\infty$ in the sense that:
\begin{align*}
\Csc^S_0 = \Big\{ 
\Wsc \Big| \sum_{l=1}^{L} ||\Wsc_l||_0 \leq S 
\Big\},
\quad 
\Csc^B_\infty = \Big\{ 
\Wsc \Big| \max_{l} ||\Wsc_l||_\infty \leq B, \; B \leq 1 
\Big\}.
\end{align*}
As a result, we denote the class of \gls{ReLU} neural networks with depth $L$, width $K$, sparsity constraint $S$ and norm constraint $B$ as $\Fsc(L, K, S, B)$, where:
\begin{align}
\Fsc(L, K, S, B) = \Big\{ f(\bx) = b_0+\beta^\top \big[ \circ_{l=1}^L (\sigma \Wsc_l) \circ x\big]  \Big| \Wsc \in \Csc^S_0, \Wsc \in \Csc^B_\infty \Big\}.
\label{eq:relu_nn}
\end{align}
When it is clear from the context, we shall use the short-hand notation $\Fsc$ for $\Fsc(L, K, S, B)$.


\subsubsection*{\gls{ReLU} Neural Network in Matrix Notation}

Given a sample $\{y_i, \bx_i\}_{i=1}^n$, the neural network predictions $\bdf_{n \times 1} = [f(\bx_1), \dots, f(\bx_n)]^\top$ 
can be represented as a $n \times 1$ vector in terms of its weight matrices. This matrix representation is mathematically convenient and provides important insight into how the data flow through the layers to interact with different components of the model. Interestingly, under the \gls{ReLU} activation function, $\bdf_{n \times 1}$ can be written as a linear product of model weight matrices despite the fact that $f(\bx)$ itself is an nonlinear model. %As a result, deep \gls{ReLU} networks share certain nice properties with the linear model. 
To keep the notation simple, in this section we will omit the bias term $b_0$. However we note that it can always be added back to the model by augmenting the feature matrix $\bPhi_{n \times K}$ (defined below) with a column vector of 1's.


We first consider the one-layer \gls{ReLU} network $f(\bx)=\beta^\top \sigma(\Wsc_1\bx)$. For a single hidden unit, the \gls{ReLU} activation output is $\sigma(\Wsc_{1,k}\bx) = I(\Wsc_{1,k}\bx > 0)*\Wsc_{1,k}\bx$, and the \gls{ReLU} output of the entire $K$-unit hidden layer is a $K \times 1$ vector $\sigma(\Wsc_1\bx) = S_{1, \bx}\, \Wsc_1\bx$, where $S_{1,\bx}$ is a $K \times K$ diagonal matrix with indicator functions $I(\Wsc_{1, k}\bx > 0)$ on the diagonal. As a result, the one-layer \gls{ReLU} network evaluated at a single observation $\bx_i$ is:
\begin{align*}
f(\bx_i) = \beta^\top S_{1,\bx_i} \Wsc_1 \bx_i.
\end{align*}
To express $\bdf_{n \times 1} = [f(\bx_1), \dots, f(\bx_n)]^\top$, we define data matrix $\bX$, weight matrix $\bW_1$ and activation matrix $\bS_{1}$ such that:
\begin{align}
\bdf_{n \times 1} = \bPhi_\Wsc\bbeta = (\bX\bW_1\bS_1)\bbeta,
\label{eq:single_layer_matrix}
\end{align}
where we have defined $\bPhi_{_\Wsc, n \times K} = \bX\bW_1\bS_1$ the matrix of hidden features, and 
\begin{align*}
\bX = 
\begin{bmatrix}
\bx_1 & 0 & \dots & 0\\
0 & \bx_2 & \dots & 0\\
\dots \\
0 & 0 & 0 & \bx_n\\
\end{bmatrix}_{n \times nP}, 
\quad
\bW_1 = \Wsc_1 \otimes \bI_n = 
\begin{bmatrix}
\Wsc_1 & 0 & \dots & 0\\
0 & \Wsc_1 & \dots & 0\\
\dots \\
0 & 0 & 0 & \Wsc_1\\
\end{bmatrix}_{nP \times nK}, 
\quad
\bS_{1} = 
\begin{bmatrix}
S_{1, \bx_1} \\ S_{1, \bx_2} \\ \vdots\\
\dots \\ S_{1, \bx_n}
\end{bmatrix}_{nK \times K}.
\end{align*}

To express $\bdf_{n \times 1}$ for a deep \gls{ReLU} network $f(\bx) = \beta^\top (\sigma \Wsc_L \dots (\sigma \Wsc_{1}\bx))$, we notice a $L$-layer \gls{ReLU} neural network evaluated at a single observation is expressed as:
\begin{align*}
f(\bx) =  \beta^\top (\prod_{l=L}^1 S_{l,\bx}\Wsc_l) \; \bx
\end{align*}
using the short-hand notation $\prod_{l=L}^1 M_l = M_L M_{L-1} \dots M_{2} M_1$. Here $S_{l, \bx}$ is a $K \times K$ diagonal matrice with indicator functions $I(\Wsc_{l,k} \sigma \Wsc_{l-1} \dots \sigma \Wsc_{1}\bx > 0)$ on the diagonal. As a result:
\begin{align}
\bdf_{n \times 1} 
= \bPhi_\Wsc\beta
= \Big( \bX (\prod_{l=1}^L \bW_l\bS_l) \Big) \beta,
\label{eq:multi_layer_matrix}
\end{align}
where $\bPhi_{\Wsc, n \times K} = \bX (\prod_{l=1}^L \bW_l\bS_l)$ is the matrix of hidden features at the output layer, and we have denoted $\bW_l = \Wsc_l \otimes \bI_n$ and $\{\bS_l\}_{l=1}^{L-1}$, $\bS_L$ as:
\begin{align*}
\bS_l = 
\begin{bmatrix}
S_{l, \bx_1} & 0 & \dots & 0\\
0 & S_{l, \bx_2} & \dots & 0\\
\dots \\
0 & 0 & 0 & S_{l, \bx_n}\\
\end{bmatrix}_{nK \times nK},
\quad
\bS_{L} = 
\begin{bmatrix}
S_{L, \bx_1} \\ S_{L, \bx_2} \\ \vdots\\
\dots \\ S_{L, \bx_n}
\end{bmatrix}_{nK \times K}.
\end{align*}

It is worth noting that the gradient function of a \gls{ReLU} network $\partial_p\bdf_{n \times 1}=[\deriv{x_p}f(\bx_1), \dots, \deriv{x_p}f(\bx_n)]^\top$ can also be expressed as a linear product of matrices. Specificially, since \gls{ReLU} network is expressed as $\bdf = \bPhi\beta$ with $\bPhi=\bX(\prod_{l=1}^L\bW_l\bS_l)\beta$, its derivative can be written as:
\begin{align*}
\partial_p\bdf_{n \times 1}
&= (\partial_p\Phi)\beta 
= \Big( \bW_{1,p}\bS_1(\prod_{l=2}^L \bW_l\bS_l) \Big)\beta
\end{align*}
where $\bW_{1, p}$ is a $n \times nK$ matrix such that $\bW_{1, p}=  \bI_n \otimes \Wsc_{1,p}$. Correspondingly, the empirical norm of the gradient function can be written as:
\begin{align*}
\psi_{p}(f) 
&= ||\deriv{x_p}f||_n^2 
= \frac{1}{n} ||\partial_p\bdf_{n \times 1}||_2^2
= \frac{1}{n}\beta^\top(\partial_p\Phi)^\top(\partial_p\Phi)\beta,
\end{align*}
which is of a quadratic form with respect to a $K \times K$ ``gradient kernel matrix" $(\partial_p\Phi)^\top(\partial_p\Phi)$.

\subsubsection*{\gls{ReLU} Network in the \gls{RKHS}}

It is important to notice that the function space $\Fsc(L, K, S, B)$ corresponds to a \glsfirst{RKHS} \citep{berlinet_reproducing_2003, bach_breaking_2014}. Specifically, notice that if we focus on the output layer, then every $f \in \Fsc(L, K, S, B)$ can be written as 
$$f(\bx) = \phi_\Wsc(\bx)^\top\beta = \sum_{k=1}^K \beta_k \phi_k(\bx|\Wsc),$$ 
where $\phi_k(\bx|\Wsc)= \Wsc_{k,L}\Big[ \circ_{l=1}^{L-1} (\sigma \Wsc_l)\circ \bx \Big]$ are the $K$ ``basis functions" at the output layer that are formed by the hidden neurons.

Consequently, $\Fsc(L, K, S, B)$ corresponds to a \gls{RKHS} $\Hsc$ equipped with positive definite kernel $k_{\Wsc}(\bx, \bx') = \phi_\Wsc(\bx)^\top\phi_\Wsc(\bx')= \sum_{k=1}^K \phi_k(\bx|\Wsc)\phi_k(\bx'|\Wsc)$, and the hidden weights $\Wsc$ can be regarded as the hyper-parameters for this \gls{RKHS} kernel  \citep{berlinet_reproducing_2003}. For two functions in this \gls{RKHS} $f(\bx)=\phi_\Wsc(\bx)^\top\beta_f$ and $g(\bx)=\phi_\Wsc(\bx)^\top\beta_g$, the inner product in $\Hsc$ is defined as:
\begin{align*}
\inner{f}{g}_{\Hsc} = \beta_f^\top\beta_g,
\end{align*}
i.e., we can interpret the output-layer weights $\beta$ as a ``representer" of $f$ in $\Hsc$. It is important to verify that the above definition of $\inner{.}{.}_\Hsc$ indeed gives rise to the  reproducing property:
\begin{align*}
\inner{f}{k(\bx, .)}_{\Hsc} = \beta_f^\top \phi_\Wsc(\bx) = f(\bx),
\end{align*}
which can be seen easily by noticing that $k_{\Wsc}(\bx, .) = \phi_\Wsc(\bx)^\top\phi_\Wsc(.)$ is an element in $\Hsc$ with its ``$\beta$" being $\phi_\Wsc(\bx)$.
Finally, the quadratic norm in this space is defined by $||f||^2_{\Hsc} = \sum_{k=1}^K \beta_{f, w}^2 = ||\beta_f||_2^2$ \citep{bach_breaking_2014}. 

To compute the kernel function $k_{\Wsc}$ and the corresponding kernel matrix $\bK_{\Wsc}$ for a \gls{ReLU} network, we recall that, for the single-layer \gls{ReLU} network $f(\bx)=\beta \sigma(\Wsc_1\bx)$, the corresponding basis function is a $K \times 1$ vector $\phi_\Wsc(\bx)_{K \times 1}=\sigma(\Wsc_1\bx) = S_{1,\bx}\Wsc_1\bx$. so we can write $k_{\Wsc}$ in terms of $\phi_\Wsc$ as:
\begin{align*}
k_\Wsc(\bx, \bx') 
&= \phi_\Wsc(\bx)^\top\phi_\Wsc(\bx') 
=
\bx^\top\Wsc_{1}^\top S_{1, \bx} \; S_{1, \bx'}\Wsc_1\bx'.
\end{align*}
Similarly, $k_{\Wsc}$ for a $L$-layer \gls{ReLU} network is:
\begin{align*}
k_\Wsc(\bx, \bx') 
= \phi_\Wsc(\bx)^\top \phi_\Wsc(\bx') 
= \bx^\top (\prod_{l=L}^1 S_{l,\bx}\Wsc_l)^\top (\prod_{l=L}^1 S_{l,\bx'}\Wsc_l) \bx'.
\end{align*}

To express the kernel matrix $\bK_{\Wsc, n \times n}$, recall the matrix of basis functions $\bPhi_{\Wsc, n \times K} = [\phi_\Wsc(\bx_1), \dots, \phi_\Wsc(\bx_n)]^\top$ can be expressed compactly as $\bPhi_\Wsc = \bX\bW_1\bS_1$ for a single-layer network, and $\bPhi_{n \times K} = \bX (\prod_{l=1}^L \bW_l\bS_l)$ for a deep \gls{ReLU} network. So the kernel matrices $\bK_{\Wsc}$ for a single-layer and a deep \gls{ReLU} network are, respectively:
\begin{align*}
\bK_{\Wsc} &= \bPhi\bPhi^\top = \bX\bW_1\bS_1\bS_1^\top\bW_1^\top\bX^\top,
\quad
\bK_\Wsc = \bPhi\bPhi^\top = \bX (\prod_{l=1}^L \bW_l\bS_l)(\prod_{l=1}^L \bW_l\bS_l)^\top \bX^\top.
\end{align*}

==> sections/background_reg.tex <==
\subsection{Problem Setup: Nonparametric Regression}

We consider a classic nonparametric regression setup, where data $\{y_i, \bx_i\}_{i=1}^n$ are observed from a data-generation distribution $P^*(y|\bx)$ for $y \in \real$ a scalar-valued response  and $\bx \in \Xsc=(0, 1)^P$ a $P \times 1$ vector of covariates  satisfying:
\begin{align*}
y_i = f^*(\bx_i) + \epsilon_i, 
\qquad \mbox{where} \qquad
\epsilon_i \sim N(0, \sigma^2).
\end{align*}
Here $f^*$ is an unknown continous function belonging to certain function class $\Fsc^*$, and $\epsilon_i$ are \gls{iid} realizations of a Gaussian white noise variable $\epsilon$ with known variance $\sigma^2$. The data dimension $P$ is allowed to be large but assumed to be $o(1)$, i.e. does not increase with the sample size $n$.

The purpose of regression is to estimate $f^*$ based on $\{y_i, \bx_i\}_{i=1}^n$ by constructing a statistical model $f:\Xsc\rightarrow \real$ that represents a certain class of functions $\Fsc$, and correspondingly, a class of model distributions $\Psc=\{P_f = N(f, \sigma^2)| f \in \Fsc\}$. We will call $\Fsc$ the model space, and denote $f_0$ the ``best" approximation of $f^*$ in $\Fsc$, in the sense that $f_0$ minimizes the \gls{KL} metric $KL(f^*, f)=E_{P^*}\big(log (P_f/P^*)\big)$. 
\footnote{The uniqueness of the \gls{KL}-projection $f_0$ is guaranteed by the fact that $\Fsc(L, K, S, B)$ is convex, i.e. any convex combination of two neural network functions $f, f' \in \Fsc$ still belongs to $\Fsc$}
\begin{comment}
For a target $f^*$, the art of nonparametric model building lies in specifying a properly-sized $\Fsc$ so that its estimator $\hat{f}$ exhibits excellent bias-variance trade-off. That is, $\Fsc$ should be rich enough so the approximation error (i.e. bias) $||f_0 - f^*||_2^2$ is small, and at the same time be sufficiently structured so the estimation error (i.e. variance) $E_{P^*}(||\hat{f} - f_0||_n^2)$ is not too high.
\end{comment}
Recent theoretical developement and empirical evidence suggests that the model space $\Fsc$ spanned by a (properly configured) deep \gls{ReLU} network achieves  excellent approximation performance for a wide class of $f^*\in \Fsc^*$ \citep{yarotsky_error_2016, schmidt-hieber_nonparametric_2017, montanelli_new_2017, suzuki_adaptivity_2018, gribonval_approximation_2019}. Therefore in this work, we focus our analysis on the Bayesian \gls{ReLU} networks' behavior in learning $f_0 \in \Fsc$, making an assumption throughout that the \gls{ReLU} model is properly configured such that $f_0 \in \Fsc$ is either identical to $f^*$ or can approximate $f^*$ with negligible error. \jzl{mention that we discuss the issue of misspecification in the end}


Given the model space $\Fsc$, the Bayesian approach to nonparametric regression is to first defining a prior distribution $\Pi: \Fsc \rightarrow [0,1]$ that assigns probability to every possible $f \in \Fsc$, and then perform learning by computing the posterior likelihood of each candidate $f$ given data $\{\bx_i, y_i\}_{i=1}^n$:
\begin{align*}
\Pi_n(f \in A) = \Pi(f \in A |\{\bx_i, y_i\}_{i=1}^n ) = 
\frac{\int_{f \in A} e^{l_n(f)} d\Pi(f)} {\int e^{l_n(f)} d\Pi(f)}
\end{align*}
where $\Pi_n(.) = \Pi(.|\{\bx_i, y_i\}_{i=1}^n)$ is the posterior distribution, and $l_n(f) = \sum_{i=1}^n l(y_i |\bx_i, f)$ is the sum of log likelihood functions over the observations $\{\bx_i, y_i\}_{i=1}^n$. 



==> sections/discussion.tex <==
\subsection{Effect of Prior Distribution on Asymptotic Distribution}


\subsection{Robustness against Model Misspecification}
\label{sec:misspec}

Mean misspecification?
\begin{enumerate}
\item vanishing approximation error.
\begin{itemize}
\item Posterior Consistency

\jzl{comment on the misspecified case of $f^* \not\in \Fsc$, the rate will be slower due to decreased approximate rate $O(n^{-(\beta-1)/d})$ \citep{xie_errors_2010}.}

\jzl{Concentration rate is not slower than that for $\Pi_n(f)$. Additional effort needed to investigate approximation error $|\psi(f) - \psi(f^*)|$ for specific function classes. This involves making technical assumptions on the smoothness and magnitude of the gradient function $\deriv{x_p}f^*$
\citep{mukherjee_learning_2006, yang_model-free_2016}, as well as 
neural network's ability in approximating gradient function (e.g. convergence result \citep{gallant_learning_1992}, approximation error rate $O(n^{-1/2d})$ \citep{hornik_degree_1994, attali_approximations_1997}, improved approximation rate $O(n^{-(\beta-1)/d})$ \citep{xie_errors_2010}) leave for future work.}
\item Uncertainty Quantification

\jzl{comment on this is a result for $f_0 \in \Fsc$ (adaptivity is not an issue since restriction on $B$ and $K$). If $f^* \not\in \Fsc$, need additional condition on prior distribution for weights to ensure the posterior of the hidden weight concentrate on a "good" set in which the convergence toward $f^*$ is $\sqrt{n}$. See, e.g., Proposition 1 in the Supplementary of  \cite{castillo_bernsteinvon_2015}. }

\jzl{
More specifically, such prior condition is of the form $\Pi(||f - f_0||_2^2 \leq C \epsilon_n) \geq exp(-n\epsilon_n)$ for the desired $\epsilon_n=O(K \,log(n)/n)$.
\citep{ghosal_convergence_2000}. Notice by \cite{vladimirova_understanding_2019}, the prior of feedforward network with $L$ layer and Gaussian prior is sub-Weibull(L/2), i.e. $\Pi(||f - f_0||_2^2 \geq C\epsilon_n) \leq a*exp(-\epsilon_n^{-1/L})$. Entropy condition can be verified using Lemma 5 of \citep{schmidt-hieber_nonparametric_2017}.}
\end{itemize}
\item nonvanishing approximation error.
\end{enumerate}

Distribution misspecification

\jzl{ add misspecification consistency theorem here}.
\citep{kleijn_misspecification_2006}
\citep{kleijn_bernstein-von-mises_2012}

\subsection{Uncertainty Quantification for Adaptive Models}



==> sections/experiment_learning.tex <==
We first empirically validate the two core theoretic results of this paper: posterior convergence (Theorem \ref{thm:post_convergence}) and the Bernstein-von Mises theorem (Theorem \ref{thm:bvm} - \ref{thm:bvm_mvn}). 
We first compare the Bayesian \gls{ReLU} network's convergence behavior in learning both $f$ and $\psi_p(f)$ under increasing sample sizes, and study how such behavior is impacted by the dimensionality of the dataset and the complexity of the data-generating function. We then verify the existence of \gls{BvM} phenonmenon for the posterior distribution $\Pi_n\big(\psi_p(f)\big)$ posterior under different combinations of  sample sizes and data dimension (Theorems \ref{thm:bvm} - \ref{thm:bvm_mvn}), thereby establishing empirical evidence for the validity of using credible interval of $\psi_p(f)$ as a rigorous tool for uncertainty quantification. Throughout the experiments, we use the standard \gls{iid} Gaussian prior for model weights, and perform posterior inference using \gls{HMC} with an adaptive step size scheme \citep{andrieu_tutorial_2008} and with 5000 burn-in iterations.

\subsubsection{Learning Accuracy and Convergence Rate}

We generate data under the Gaussian noise model $y \sim N(f^*, \sigma^2=1)$ for data-generation function $f^*: [0, 1]^{d^*} \rightarrow \real$ with true dimension $d^* = 5$. For the input features $\bX_{n \times d}$, we generate from uniform distribution as $x_{i, j} \stackrel{i.i.d.}{\sim} U(0, 1)$ for sample sizes $n \in (100, 2000)$, and vary data dimension between $d \in (25, 200)$ to cover high-dimension cases such as $n=100, d=200$. For the neural network model, we consider a 2-layer, 50-hidden-unit feedforward network (i.e., $L=2$ and $K = 50$) that is typically used in practice.

We consider three different data-generation functions $f^*$ that are increasingly difficult for an neural network to approximate: (1) \textbf{linear}, i.e., a simple linear model $f^*(\bx) = \bx^\top \bbeta$, (2) \textbf{neural}, i.e., a function $f^* \in \Fsc(L, W, S, B)$ sampled from the neural network's model space, and (3) \textbf{complex}, i.e., a complex, non-smooth multivariate  function:
\begin{align*}
f^*(\bx) &= \frac{sin(max(x_1, x_2)) + arctan(x_2)}{1 + x_1 + x_5} + sin(0.5 \, x_3) \big(1 + exp(x_4 - 0.5 \, x_3) \big) + x_3^2 + 2 \, sin(x_4) + 4 \, x_5.
\end{align*}
Notice that while the \textbf{linear} and \textbf{neural} functions belong to $\Fsc(L, W, S, B)$, the third function (\textbf{complex}) does not fall exactly in $\Fsc(L, W, S, B)$ \footnote{For example, $f^*$ is non-continous in terms of $x_1, x_2$, but is infinitely differentiable in terms of $x_3, x_4, x_5$} but can be approximated with decreasing error in a nonparametric rate \citep{schmidt-hieber_nonparametric_2017}. Therefore the \textbf{complex} function serve as a case to examine whether the posterior convergence still holds when $f^* \not\in \Fsc$.

For each setting of $(n, d, f^*)$, we repeat the simulation 20 times and evaluate the neural network's performance in learning $f$ and $\psi_p(f)$ using out-of-sample standardized \gls{MSE} against $f^*$ and $\psi(f^*)$:
\begin{align*}
std\_MSE(f, f^*) = 
\frac{\frac{1}{n}\sum_{i=1}^n (f(\bx_i) - f^*(\bx_i))^2}
{\frac{1}{n}\sum_{i=1}^n( f^*(\bx_i) - \bar{f}^*(\bx_i))^2},
\end{align*}
and $std\_MSE$ for $\psi(f)$ is computed similarly and is averaged over all $p$. Notice that $std\_MSE$ is essentially $1$ minus the $R^2$ statistic that is used to measure the model's goodness-of-fit in regression modeling, it is standardized between $(0, 1)$ and therefore allows direct comparison of model performance across different $f^*$'s.

\begin{figure}[ht]
    \centering
    \subfloat{\includegraphics[width=0.33\textwidth]{"./figure/learning_pred_linear"}}
    \subfloat{\includegraphics[width=0.33\textwidth]{"./figure/learning_pred_neural"}}
    \subfloat{\includegraphics[width=0.33\textwidth]{"./figure/learning_pred_barron"}}
    
    \subfloat{\includegraphics[width=0.33\textwidth]{"./figure/learning_var_imp_mean_linear"}}
    \subfloat{\includegraphics[width=0.33\textwidth]{"./figure/learning_var_imp_mean_neural"}}
    \subfloat{\includegraphics[width=0.33\textwidth]{"./figure/learning_var_imp_mean_barron"}}
\caption{BNN's convergence behavior for learning prediction $f^*$ (first row) and variable importance $\psi(f^*)$ (second row)  under sample sizes $n \in (100, 2000)$ for $d \in (50, 200)$. Column 1-3 corresponds to \textbf{linear}, \textbf{neural}, and \textbf{complex}.}

\label{fig:learning}
\end{figure}

Figure \ref{fig:learning} summarizes the standardized \gls{MSE}s for learning $f^*$ and $\psi(f^*)$, where the first and second row corresponds to $std\_MSE$'s for $f^*$ and $\psi(f^*)$, and each column corresponds to a data-generation machanism (\textbf{linear}, \textbf{neural} and \textbf{complex}). We first examine model performance in prediction (i.e., in learning $f^*$) across different data-generation mechanisms by inspecting the first row. The model performance in prediction shows strong pattern of the \textit{curse of dimensionality}, as the model's prediction performance clearly deteriorates as the data dimension increases. Interestingly, the models' converge behavior for \textbf{linear} and \textbf{neural} are observed to be similar, despite the former being a much simpler function. This suggests that the model's prediction performance is sufficiently fast for any $f^* \in \Fsc$ that belongs to the model space. Comparatively, we observe that the model error for \textbf{complex} is higher and converges to zero in a slower rate, due to the fact that $f^* \not\in \Fsc$. (Note that this does not suggest that the model estimate for \textbf{complex} is biased, since by the the universal approximation property, the model error of a neural network will eventually decreases to zero).

We next examine the relation between model's convergence behavior  in learning $f^*$ (first row) and in learning $\psi(f^*)$ (second row). Comparing to the model's learning speed in prediction, we observe that the model's learning speed for variable importance is in fact much faster and less susceptible to the curse of dimensionality. This verifies our conclusion in Theorem \ref{thm:post_convergence} that a model's good behavior in prediction translates to good performance in learning variable importance. We also observe that when the theorem assumption $f^* \in \Fsc$ is violated (e.g. for \textbf{complex} $f^*$ on Column 3), the posterior convergence still occur albeit at a slower rate.

\subsubsection{Bernstein-von Mises Phenonmenon}
We next verify the Bernstein-von Mises phenonmenon for the variable importance posterior $\Pi_n \big(\psi_p(f)\big)$. For this set of experiment, we increase the range of sample size to $n \in (100, 10000)$ and reduce layer size to $L = 1$ to save computation time.

We evaluate the model's convergence behavior toward the asymptotic posterior $N(0, 4||H_p \, f_0||_n^2)$ using two metrics: (1) the standardized \gls{MSE} of posterior standard deviation (which is expected to converge to $\frac{2}{\sqrt{n}}||H_p f_0||_n$). We use this metric to assesses whether the spread of the posterior distribution (and correspondingly the credible interval) is correct. (2) The \gls{CvM} statistic (i.e. the empirical $L_2$ distance) between the posterior sample and a Gaussian distribution. We use this statistic to assess whether the shape of the posterior distribution is sufficiently symmetric. Specifically, to compute the CvM metric given $M$ posterior samples of the centered variable importance $\{\psi^c_m\}_{m=1}^M$, we compute the standardized variable importance as $\psi^c_{std, m}=\hat{\Sigma}^{-1/2}\big(\psi^c_m - \hat{E}(\psi^c)\big)$, and then compute \gls{CvM} statistic as the $L_2$ distance between the empirical \gls{CDF} $\Fbb(\psi_{std})$ and a Gaussian \gls{CDF} $\Phi$:
\begin{align*}
CvM(\Fbb, \Phi) = 
\frac{1}{M}\sum_{m=1}^M \big[\Fbb(\psi^c_{std, m}) - \Phi(\psi^c_{std},m)\big]^2
\end{align*}
If $\Pi_n(\psi^c)$ is multivariate Gaussian, then $\psi^c_{std}$ is expected to follow a standardized Gaussian distribution, leading to a \gls{CvM} with small value. Notice that since the \gls{CvM} statistic can never be zero, we assess whether $\hat{\Sigma}^{-1/2}\big(\psi - \hat{E}(\psi)\big)$ is sufficiently Gaussian by comparing its CvM statistic to a null distribution where $\Fbb$ is computed from a Gaussian random sample of the same size.

\begin{figure}[ht]
    \centering
    \subfloat{\includegraphics[width=0.45\textwidth]{"./figure/uq_std_r2_neural"}}
~    
    \subfloat{\includegraphics[width=0.45\textwidth]{"./figure/uq_cvm_neural_full"}}
\caption{The variable importance posterior's convergence behavior toward the asymptotic standard deviation (left, measured by standardized \gls{MSE}) and toward normality (right, measured by the \gls{CvM} distance from a Gaussian distribution) under sample size $n \in (100, 10000)$ and $d \in (25, 100)$. Shaded region in the right figure indicates the $\{5\%, 10\%, 25\%, 75\%, 90\%, 95\%\}$ quantiles of the null CvM distribution.}
\label{fig:uq}
\end{figure}

Figure \ref{fig:uq} summarizes the result. The variable importance posterior $\Pi_n \big(\psi^c(f) \big)$'s convergence behavior in standard deviation (measured by $std\_MSE$) and in normality (measured by $CvM$) are shown on the left and right figures, respectively. The shaded region in the right figure indicates the $\{5\%, 10\%, 25\%, 75\%, 90\%, 95\%\}$ quantiles of the null CvM distribution. As shown, as the sample size increases, the standardized \gls{MSE} for $sd(\psi^c)$ converges toward 0, and the \gls{CvM} statistics enters into the range of the null distribution, with the speed of convergence deteriorates (although not very dramatically) as the data dimension increases. Above observations indicates that the credible intervals from the variable importance posterior $\Pi_n \Big(\psi^c(f) \Big)$ indeed achieve the correct spread and shape in reasonably large sample as suggested by the \gls{BvM} Theorems \ref{thm:bvm} - \ref{thm:bvm_mvn}. Consequently, the $(1-q)$-level credible intervals from $\Pi_n \Big(\psi^c(f) \Big)$ are valid tools for rigorous uncertainty quantification, i.e. they indeed cover the true parameter $\psi(f^*)$ for $(1-q)\%$ of the time.

==> sections/intro_full.tex <==
The advent of modern data era has given rise to voluminous, high-dimensional datasets in which the outcome has complex, nonlinear dependency on the input features. In this nonlinear, high-dimensional regime, a fundemental task behind many knowledge discovery endeavors is variable selection, i.e. to identify a small subset of features that is the most relevant in explaining the outcome. Examples abound from genome-wide association studies for causal variant \citep{buhlmann_high-dimensional_2014}, to large-scale health effect studies using electronic medical record to identify disease risk factors \citep{di_air_2017}, to profolio selection and stock price prediction in financial market \citep{fan_statistical_2007}.

Over the past few decades, a number of variable selection methods  have been developed based on various classic or machine learning models (see Section \ref{sec:lit_review} for a review). Core to these approaches is a two-step procedure: First, a model parameter is defined to encode the importance of an input variable $x_p$ in explaining the outcome (e.g. the regression coefficient $\beta_p$ under linear model $y=\sum_p x_p\beta_p$, or the gradient function norm $||\deriv{x_p}f||^2_n$ under a smooth nonlinear model $y=f(x_1,\dots,x_P)$ \citep{rosasco_nonparametric_2013}). Then, a variable-selection decision rule is devised based on the estimated variable importance. Examples of the types of decision rule include thresholding \citep{fan_sure_2008}, 
hypothesis testing \citep{lockhart_significance_2013}, or simply inspecting whether the penalized parameter estimate is zero \citep{fan_selective_2010}. Clearly, the effectiveness of the variable selection procedure depends both on the quality of the model estimator for variable importance (measured by the convergence speed toward the truth), and on the appropriateness of the decision rule for the problem at hand (e.g., whether its \gls{FDR} is properly controlled for). 

\subsection*{Challenges for Nonlinear Variable Selection in High Dimension}

The high-dimension regime brings two challenges to  nonlinear variable selection. The first challenge is the \textit{curse of dimensionality}, i.e. the exponentially increasing difficulty in estimating the variable importance parameters in the high dimension. In the context of nonparametric learning, such difficulty is often measured by the learning rate $\epsilon_n$, which describes the sample size required for an estimator to reach certain level of statistical precision $\epsilon_n$ (measured by, e.g, the $L^2$ risk) \citep{gine_mathematical_2015}. For example, for $f$ a $\beta$-times differentiable, Lipschitz-continuous functions in $\real^d$, it is well known that the optimal (minimax) rate for learning $f$ is lower bounded by $\epsilon_n = O(n^{-\frac{\beta}{2\beta + d}})$
\citep{donoho_adapting_1995, cai_rates_2003}. This implies that 
the statistical accuracy of a nonlinear model (e.g., kernel method or random forest) decays exponentially as the data dimension $d$ increases, leading to increasingly unreliable estimate of variable importance.

The second challenge is \textit{multiple comparison}, i.e., the difficulty in constructing a high dimensional decision rule that maintains the correct level of precision (e.g., 1 - false discovery rate) \citep{buhlmann_statistical_2013}. 
%A low-precision decision rule in high dimension falsely selects many irrelevant variables, leading to false discovery and consequently scientific conclusions that are not trustworthy. 
The multiple comparison problem often arise when a multivariate decision is made based purely on individual decision rules, ignoring the dependency structure among the decisions. For example, consider a ``low dimension" dataset with $100$ variables. Even with a decent selection procedure that has precision $0.95$ in selecting one variable, the probability of selecting at least one irrelevant variable out of the $100$ variable is $1 - 0.95^{100} \approx 0.994$ (assuming independence between decisions), leading to an un-trustworthy overall procedure with precision $\leq 0.006$. 
As a result, in order to be effective in high dimension, it is necessary for a variable selection procedure to have explicit control over its overall \gls{FDR}. Unfortunately, this is difficult to achieve with naive decision rules based on regularized estimates (e.g. LASSO), where the precision-recall trade-off is done implicitly by adjusting the regulization strength through the tunning parameter, and it is usually unclear how to set the the tunning parameter to control the \gls{FDR} at certain required level (e.g. $0.05$). On the other hand, in the statistics literature, there exists several multiple-comparison correction procedures including the Bonferroni correction, Bonferroni-Holm method \citep{holm_simple_1979} and the Benjamini-Hochberg procedure \citep{benjamini_control_2001}. However, most of these methods focus on adjusting the decision threshold of the marginal decision rules, not exploiting the covariance structure of the problem, and as a result, often lead to conservative variable selection conclusions with low sensitivity \citep{buhlmann_high-dimensional_2014}.


\subsection*{Bayesian Deep Learning as an Promising Solution}
To this end, the main interest of this work is to establish  Bayesian Deep Neural Network as an effective tool for tackling both of these challenges.

Deep neural network is known to be an effective model for high-dimensional learning problems, illustrating empirical success in applications such as image classification and speech recognition  where the traditional nonparametric methods (e.g. kernel methods and tree ensembles) have had limited success. Recent theoretical studies showed that the neural networks have the remarkable ability of ``breaking" the curse of dimensionality by adapting to the underlying structure of the data \citep{barron_approximation_1994, bach_breaking_2014, suzuki_adaptivity_2018, nakada_adaptive_2019}. For example, \cite{bach_breaking_2014} showed that when learning data generated by various structured models (e.g. affine function or additive nonlinear function), a neural network with one hidden layer can already avoid the exponential dimension penalty  and achieves a remark parametric rate of $\epsilon_n = O(d^\frac{1}{2} n^{-\alpha})$ for some $\alpha > 0$ not depending on dimension $d$. The similar phenonmenon is shown to hold for more general function spaces, as long as they satisfy certain smoothness property (e.g. has integrable Fourier transform \citep{barron_approximation_1994, barron_approximation_2018} or lies in a mixed smoothness Besov space \citep{suzuki_adaptivity_2018}). Improving on the shallow networks, deep neural networks with \gls{ReLU} activation are shown to have expressive power that grows exponentially with the number of layers \citep{poole_exponential_2016, raghu_expressive_2017}. This suggests the deep neural network needs much smaller number of parameters to achieve the same level of approximation accuracy \citep{lin_why_2016}. From a statistical perspective, this fact implies that the bias-variance trade-off under a deep neural network is remarkably ``economical", which leads to higher statistical efficiency and faster convergence toward the underlying data-generation function, thereby providing statistical justification for the empirical success of deep learning models.

Bayesian inference in neural networks, on the other hand, provides a principled framework for uncertainty quantification that naturally handles the multiple comparison problem \citep{gelman_why_2012}. By sampling from the joint posterior distribution of variable importance parameters, Bayesian inference provides easy access to not only the model uncertainty about the individual variables, but importantly, a complete picture of the dependency structure among all the input covariates. This information has allowed the variable selection procedures to tailor their decision rule with respect to the correlation structure of the problem, leading to a more precise and informative precision-recall trade-off in high dimension. Furthermore, if the posterior distribution for the variable importance parameters satisfies an \gls{BvM} phenomenon (i.e., asymptotic normality), then the Bayesian posterior credible intervals will automatically acquire a rigorous frequentist interpretation (e.g. a $95\%$ credible interval covers the truth $95\%$ of the time / has \gls{FDR} $0.05$) \citep{castillo_bernsteinvon_2015}. As a result, decision rules constructed under Bayesian paradigm has precise control of its overall \gls{FDR} while maintain sufficient detection power, leading to an effective variable selection procedure that is suitable for high dimensional problems.


\begin{comment}
Review of Approximation Adaptivity / Avoid curse of dimensionality
\begin{itemize}
\item General Function Space: H\"{o}lder $\Csc^\beta$ \citep{schmidt-hieber_nonparametric_2017} $\epsilon_n \asymp O\Big(n^{-\frac{\beta}{\beta + d/2}}\Big)$
\item Alleviate curse of dimensionality by making additional  assumption on either the structure or the smoothness of $f_0$:
\begin{itemize}
\item Parametric Structure \citep{bach_breaking_2014}.
\item Barron class \citep{barron_approximation_1994} 
$\epsilon_n \asymp O\Big((d / log \, n)^{\frac{1}{2}} * n^{-\frac{1}{2}}\Big)$
\item Besov and mixed Besov space $mB^\beta_{p, q}$ \citep{suzuki_adaptivity_2018}
$\epsilon_n \asymp O\Big(log\, n ^{\frac{(d-1)(\beta + u)}{\beta + 1/2}} * n^{-\frac{\beta}{\beta + 1/2}}\Big)$, where $u = (1 - \frac{1}{q})_+$ for $p \geq 2$. For example, a space of Sobelov-type (i.e. $p=q=2$) corresponds to $u = \frac{1}{2}$, for which the estimation error rate is $\epsilon_n \asymp O\Big(log\, n\,^{d - 1} * n^{-\frac{\beta}{\beta + 1/2}}\Big)$.
\end{itemize}
\end{itemize}

Finally, it is interesting to note that....

ability in gradient learning is verified ability in approximating Bernstein polynomials at a rate $O(N^{-(\beta-1)/d})$ \citep{hornik_degree_1994, attali_approximations_1997, xie_errors_2010}
\end{comment}


\subsection*{Summary of contributions}

In this work, we propose a simple variable selection method for high-dimensional regression based on credible intervals of a deep Bayesian \gls{ReLU} network. Consistent with the existing nonlinear variable selection approaches, we measure the importance of an input variable $x_p$ using the empirical norm of its gradient function $\psi_p(f)=||\deriv{x_p}f||_n^2$ \citep{white_statistical_2001, rosasco_nonparametric_2013, yang_model-free_2016, he_scalable_2018}. We perform variable selection by first computing the $(1-\alpha)$-level simutaneous credible intervals for the joint posterior distribution $\psi(f)=\{\psi_p(f)\}_{p=1}^P$, and then make variable-selection decision by inspecting whether the credible intervals includes 0. The salient features of this method includes sparsistent variable selection that is powerful in high dimension (due to the use of deep neural network), and the ability to precisely control over its operating characteristics such as the \gls{FDR} (due to the use of Bayesian method). It is easy to implement, computationally efficient, agnostic to model architecture and is compatible with a wide range of prior choices.

To set the method on a solid theoretical footing, we establish two new Bayesian nonparametric results to answer below two questions: (1) does the neural network's optimal performance in high-dimensional prediction translates to that in learning variable importance? (2) Do the variable-selection decision rules constructed using Bayesian credible intervals have a valid frequentist interpretation, e.g., do decisions based on the $(1-\alpha)$-level credible intervals guarantee a \gls{FDR} of $\alpha$ under the true data-generation mechanism $P_0$? To this end, we develope a complete set of Bayesian nonparametric theorems that are  important for understanding the deep \gls{ReLU} neural networks' behavior in learning $\psi(f)$. They include:

\begin{enumerate}
\item \textbf{Posterior Consistency and Non-asymptotic Contraction Rate}. For a properly configured \gls{ReLU} network with learning rate $\epsilon_n$, the entire posterior distribution of $\psi(f)$ (the variable importance parameters) concentrates toward the truth in a speed no slower than $\epsilon_n$, i.e. neural network is effective  in learning variable importance in high dimension (Theorem \ref{thm:post_convergence}). In the context of the proposed variable selection algorithm, this result endows our procedure an important property known as  \textit{sparsistency}, i.e., the procedure asymptotically eliminates the irrelevant variables and recovers the set of truely informative variables with probability 1 \citep{ravikumar_sparse_2007} (Theorem \ref{thm:sparsistency}).


\item \textbf{\glsfirst{BvM} Theorem} (i.e. asymptotic normality). More importantly, we develope a semi-parametric \glsfirst{BvM} theorem for deep \gls{ReLU} network model in learning the multivariate nonlinear functional $\psi(f)=\{||\deriv{x_p}f||^2_n\}_{p=1}^P$ (Theorem \ref{thm:bvm} and \ref{thm:bvm_mvn}). The \gls{BvM} theorem asserts that the posterior distribution of $\psi(f)$ is asymptotically normal, and that the uncertainty quantification using the neural network posterior is rigourous, in the sense that a $95\%$ credible interval indeed covers the true parameter $95\%$ of the time (i.e. correct frequentist coverage) \citep{castillo_bernsteinvon_2015}. In the context of the proposed algorithm, this result has the important implication that variable selection based on the $(1-\alpha)$-level \textit{simutaneous} credible interval indeed lead to a variable selection procedure with overall precision $1-\alpha$ (or \gls{FDR} $\alpha$). To authors' knowledge, this is the first semi-parametric \gls{BvM} result for deep neural network models.
\end{enumerate}

The rest of the paper is organized as follows. After reviewing the related literature in Section \ref{sec:lit_review}, Section \ref{sec:background} sets up the nonparametric regression problem  and introduce necessary background on Bayesian neural networks, specifically about its representation as a (conditional) \gls{GP} in a \gls{RKHS}. The main theoretical results are specialized in Section \ref{sec:theory}, where we introduce the variable importance measure $\psi(f)$ and establishes its posterior consistency and \gls{BvM} phenonmenon under the deep \gls{ReLU} neural network. Section \ref{sec:algorithm} formally present the proposed variable selection algorithm, establishing its sparsistency property, and discusses the computational details. The numerical experiments on the simulated examples and real applications are contained in Section \ref{sec:exp}.  A brief discussion is provided in Section \ref{sec:discussion},  and the Appendix is devoted to the technical proofs.



==> sections/keywords.tex <==
\vspace{1em}

\begin{keywords}
Bayesian Neural Network. Deep Learning. High-dimensional Statistics, Feature Selection. Uncertainty Quantification. Posterior Convergence. Bernstein-von Mises Theorem
\end{keywords}


==> sections/method_def.tex <==
\subsection{Measure Variable Importance using Gradient Norm}
\label{sec:var_imp}

In nonlinear modeling for a smooth function $f:\real^P \rightarrow \real$, the importance of a variable $x_p$ in influencing the outcome $y=f(\bx)$ at a point $\bx_i$ is captured by the magnitude of the corresponding partial derivative $\big| \deriv{x_p} f(\bx_i) \big|$ \citep{wahba_spline_1990, rosasco_nonparametric_2013, he_scalable_2018}. Therefore, to summarize the overall importance of a variable $x_p$ over the entire feature space $\bx \in \Xsc$, a natural measure is:
\begin{align}
\Psi_p(f) &=
\Big|\Big| \deriv{x_p} f \Big|\Big|_{2}^2 = 
\int_{\bx \in \Xsc} \Big| \deriv{x_p} f(\bx) \Big|^2 dP(\bx).
\label{eq:var_imp_2_norm}
\end{align}
where $P(\bx)$ is the marginal probability measure of input covariates $\bx \in \Xsc$. Given observations $\{\bx_i, y_i\}_{i=1}^n$, a natural empirical proxy of $\Psi_p(f)$ is:
\begin{align}
\psi_p(f) &=
\Big|\Big| \deriv{x_p} f \Big|\Big|_n^2 = 
\frac{1}{n}\sum_{i=1}^n \Big| \deriv{x_p} f(\bx_i) \Big|^2.
\label{eq:var_imp_n_norm}
\end{align}
Notice that $\psi_p: \Hsc \rightarrow \real$ is a scalar-valued parameter that depends on the target function $f$, rather than a summary  statistic that is completely determined by the data.

Under a \gls{ReLU} neural network, computing $\psi_p(f)$ is simple due to the property of \gls{ReLU} activation function. Specifically, for a $L$-layer \gls{ReLU} network $f(\bx)=\beta (S_{L,\bx} \Wsc_L \dots (S_{1,\bx} \Wsc_{1}\bx ))$, the corresponding derivative function $\psi_p(f)$ is:
\begin{align}
\psi_p(f) &= \sum_{i=1}^n \Big|\deriv{x_p} f(\bx_i)\Big|^2
\quad \mbox{where} \quad
\deriv{x_p} f(\bx) 
= 
\beta \Big(S_{L,\bx} \Wsc_L \dots \big(S_{1,\bx} \Wsc_{1,p} \big)\Big),
\label{eq:nn_grad}
\end{align}
where $\Wsc_{1,p}$ is the $p^{th}$ column of the input-layer hidden weights $\Wsc_1$. Note that the expression of $\deriv{x_p} f(\bx)$ is similar to that of $f(\bx)$, except with the  input features $\bx$ and non-$p$ input weights in $\Wsc_1$ removed. This suggests that the behavior of the gradient function $\deriv{x_p}(f)$ could be similar to that of $f(\bx)$. In practice, $\deriv{x_p} f(\bx)$ can be computed easily for neural networks using standard automatic differentiation libraries, e.g., TensorFlow \citep{abadi_tensorflow:_2016}.



==> sections/proof/Hp_norm.tex <==
Notice that $||\bH_p||_2 = O_p(1)$ implies $tr(\bH_p)=O_P(K)$ since  
$$tr(\bH_p) \leq rank(\bH_p) * ||\bH||_2 = O_p(rank(\bH_p)) = O_p(K).$$ Therefore we only need to show $||\bH||_2 = O_p(1)$.

Show $||\bH_p||_2 = O_p(1)$ by showing that it is upper bounded by certain constant that does not depend on $n$. Recall that $\bH_p = (\bPhi^+)^\top(\partial_p\bPhi^\top \partial_p\bPhi)\bPhi^+$, by the fact that 2-norm is invariant under cyclic permutations, we then have 
\begin{align*}
||\bH_p||_2 
&= ||(\partial_p\bPhi\bPhi^+)^\top(\partial_p\bPhi\bPhi^+)||_2
= ||\partial_p\bPhi(\bPhi^+\bPhi^{+\top})\partial_p\bPhi^\top||_2
= ||\partial_p\bPhi(\bPhi^\top\bPhi)^{-1}\partial_p\bPhi^\top||_2\\
&= ||(\bPhi^\top\bPhi)^{-1}(\partial_p\bPhi^\top\partial_p\bPhi)||_2
\end{align*}

Denote $\bM=\bS_1(\prod_{l=2}^L \bW_l\bS_l)$, then we have $\bPhi = \bX\bW_1\bM$ and $\partial_p\bPhi = \bW_{1, p}\bM$. Denote $\bX_p = diag(x_{1, p}, x_{2, p}, \dots, x_{n, p})$ and notice that $\bX\bW_1 = \sum_{p}\bX_p\bW_{1, p}$, so we see that $\bPhi$ is related to $\partial_p \bPhi$ through the expression $\bPhi=\sum_p \bX_p \partial_p\bPhi$, and
\begin{align*}
\bPhi^\top\bPhi
&= (\sum_p \bX_p \partial_p\bPhi)^\top(\sum_p \bX_p \partial_p\bPhi)
=
\sum_{p_1, p_2}
\partial_{p_1}\bPhi^\top\bX_{p_1}\bX_{p_2} \partial_{p_2}\bPhi.
\end{align*}

Using the inversion formula $(\bA + \bB)^{-1} = (\bI + \bA^{-1} \bB)^{-1}\bA^{-1}$ \citep{henderson_deriving_1981}, we can write $(\bPhi^\top\bPhi)^{-1}$ as:
\begin{align*}
(\bPhi^\top\bPhi)^{-1} &= 
\Big(
\partial_{p}\bPhi^\top\bX^2_{p} \partial_{p}\bPhi + 
\sum_{p_1,p_2\neq p}
\partial_{p_1}\bPhi^\top\bX_{p_1}\bX_{p_2} \partial_{p_2}\bPhi \Big)^{-1}\\
&= 
\Big(\bI + 
(\partial_{p}\bPhi^\top\bX^2_{p} \partial_{p}\bPhi)^{-1}
\sum_{p_1,p_2 \neq p}\partial_{p_1}\bPhi^\top\bX_{p_1}\bX_{p_2} \partial_{p_2}\bPhi
\Big)^{-1} (\partial_{p}\bPhi^\top\bX^2_{p} \partial_{p}\bPhi)^{-1}.
\end{align*}
Consequently, we can bound $||\bH_p||_2$ as:
\begin{align*}
||\bH_p||_2
&= 
||(\bPhi^\top\bPhi)^{-1}(\partial_p\bPhi^\top\partial_p\bPhi)||_2
\\
&=
\Big|\Big|
\Big(\bI + 
(\partial_{p}\bPhi^\top\bX^2_{p} \partial_{p}\bPhi)^{-1}
\sum_{p_1,p_2 \neq p}\partial_{p_1}\bPhi^\top\bX_{p_1}\bX_{p_2} \partial_{p_2}\bPhi
\Big)^{-1} 
(\partial_{p}\bPhi^\top\bX^2_{p} \partial_{p}\bPhi)^{-1}(\partial_p\bPhi^\top\partial_p\bPhi)
\Big|\Big|_2
\\
&\leq \Big|\Big|
\Big(\bI + 
(\partial_{p}\bPhi^\top\bX^2_{p} \partial_{p}\bPhi)^{-1}
\sum_{p_1,p_2 \neq p}\partial_{p_1}\bPhi^\top\bX_{p_1}\bX_{p_2} \partial_{p_2}\bPhi
\Big)^{-1} 
\Big|\Big|_2 *
\Big|\Big|
(\partial_{p}\bPhi^\top\bX^2_{p} \partial_{p}\bPhi)^{-1}
(\partial_p\bPhi^\top\partial_p\bPhi)
\Big|\Big|_2
\end{align*}

Notice in the last line of the above expression, the first term can be bounded as:
\begin{align}
\Big|\Big|
\Big(\bI + 
(\partial_{p}\bPhi^\top\bX^2_{p} \partial_{p}\bPhi)^{-1}
\sum_{p_1,p_2 \neq p}\partial_{p_1}\bPhi^\top\bX_{p_1}\bX_{p_2} \partial_{p_2}\bPhi
\Big)^{-1} 
\Big|\Big|_2 &\leq 1
\label{eq:Kinv_Hp_term_1}
\end{align}
This is because $\lambda_{\min}\Big(\bI + 
(\partial_{p}\bPhi^\top\bX^2_{p} \partial_{p}\bPhi)^{-1}
\sum_{p_1,p_2 \neq p}\partial_{p_1}\bPhi^\top\bX_{p_1}\bX_{p_2} \partial_{p_2}\bPhi \Big)\geq 1$ due to the fact that $\partial_{p_1}\bPhi^\top\bX_{p_1}\bX_{p_2} \partial_{p_2}\bPhi$ is full column rank for all $p_1, p_2$, which implies that $\lambda_{\max}$ of (\ref{eq:Kinv_Hp_term_1}) is no larger than 1.

The second term can be bounded as:
\begin{align}
||(\partial_{p}\bPhi^\top\bX^2_{p} \partial_{p}\bPhi)^{-1}
(\partial_p\bPhi^\top\partial_p\bPhi)||_2 
&= 
||(\partial_{p}\bPhi^+\bX_{p}^{-2} \partial_{p}\bPhi^{+\top})
(\partial_p\bPhi^\top\partial_p\bPhi)||_2 
\nonumber\\
&= 
||\partial_{p}\bPhi^+\bX_{p}^{-2} \partial_p\bPhi||_2
\nonumber\\
&= 
||\bX_{p}^{-2} \partial_p\bPhi\partial_{p}\bPhi^+||_2
\nonumber\\
&\leq ||\bX_{p}^{-2}||_2 ||\partial_p\bPhi\partial_{p}\bPhi^+||_2 
\nonumber\\
&=||\bX_{p}^{-1}||^2_2,
\label{eq:Kinv_Hp_term_2}
\end{align}
where we have denoted $\bPhi^+ = \bV\bD^{-1}\bU^\top$ for $\bPhi = \bU\bD\bV^\top$. In above expression, the third equality follows from the fact that the eigenvalue of the product of square matrices is 
invariant under cyclic permutation of the product order
%\href{https://math.stackexchange.com/questions/281016/invariance-of-eigenvalues-of-a-product-of-square-matrices-under-cyclic-permutation}{invariant under cyclic permutation of the product order} 
\citep{merikoski_inequalities_2004}.

Combining (\ref{eq:Kinv_Hp_term_1}) and (\ref{eq:Kinv_Hp_term_2}), we have:
\begin{align*}
||\bH_p||_2
&= 
||(\bPhi^\top\bPhi)^{-1}(\partial_p\bPhi^\top\partial_p\bPhi)||_2
\\
&\leq \Big|\Big|
\Big(\bI + 
(\partial_{p}\bPhi^\top\bX^2_{p} \partial_{p}\bPhi)^{-1}
\sum_{p_1,p_2 \neq p}\partial_{p_1}\bPhi^\top\bX_{p_1}\bX_{p_2} \partial_{p_2}\bPhi
\Big)^{-1} 
\Big|\Big|_2 *
\Big|\Big|
(\partial_{p}\bPhi^\top\bX^2_{p} \partial_{p}\bPhi)^{-1}
(\partial_p\bPhi^\top\partial_p\bPhi)
\Big|\Big|_2
\\
&\leq
||\bX_p^{-1}||^2_2 
\end{align*}
Recall that since $\bX_p=diag(\bx_{1, p}, x_{2, p}, \dots, x_{n, p})$ is a diagonal matrix, we have $||\bX_p^{-1}||_2 = max(1/x_{i, p})= 1/min(x_{i, p}) \leq 1/c_x$, i.e. bounded by a constant that does not depend on $n$. Therefore $||\bH_p||_2 = O_p(1)$.


==> sections/proof/algorithm.tex <==
\subsection{Computing Variable Importance}

In this section we consider how to compute $\psi^c_p(f)$ in practice, analyze the corresponding computation complexity, and propose a parallel algorithm so the computation is scalable to large $n$ and $P$ by taking advantage of the modern multi-core architecures.

Recall that $\psi^c_p(f) = \psi_p(f) - E_0(\eta_n)$ where $\eta_n = \hat{\psi}_p - \hat{\psi}(f_0)$ is the estimator of the asymptotic bias. Notice that (\ref{eq:psi_estimator}) implies that $\eta_n = E_{P_0}(\hat{\psi}_p - \hat{\psi}(f_0)) = E_{P_0}(\frac{2}{\sqrt{n}}\inner{H_pf_0}{\omega}_n + \frac{1}{n}\inner{H_p\omega}{\omega}_n)=E_{P_0}(\frac{1}{n}\inner{H_p\omega}{\omega}_n)$. Therefore, given observation $\{\bx_i, y_i\}_{i=1}^n$, if $\epsilon$ is a zero-mean, unit-variance random variable under $P_0$, we can evaluate $E_0(\eta_n)$  as $\eta_n = E_{P_0}(\inner{H_p\omega}{\omega}_n) = E(\bepsilon^\top\bH_p \bepsilon) = tr(\bH_p)$, where recall that $\bH_p=\bD_p^\top\bD_p=(\bPhi^+)^\top\partial_p\bPhi^\top\partial_p\bPhi \bPhi^+$ for $\Phi_{n \times K}=\bX\bW_1\bS_1(\prod_{i=1}^L \bW_l\bS_l)$ and $(\partial_p\Phi)_{n \times K}=\bW_{1,p}\bS_1(\prod_{l=2}^L \bW_l\bS_l)$.

Therefore in practice, given Monte Carlo samples from the neural network posterior $\Pi_n(f, \Wsc)$, the variable importance $\psi_p^c(f)$ is evaluated as:
\begin{align*}
\psi^c_p(f) = ||  \deriv{x_p}f ||_n^2 - tr(H_p) 
&=
||\partial_p\bPhi\beta||^2_2 - tr\Big((\bPhi^+)^\top\partial_p\bPhi^\top\partial_p\bPhi \bPhi^+\Big).
%\\
%&=
%tr\Big(
%\partial_p\bPhi^\top\partial_p\bPhi (\beta\beta^\top - \bPhi^+\bPhi^{+\top}) 
%\Big).
\end{align*}
To obstain a simple expression of $\psi^c_p(f)$ that is convienient for computation, we denote $\bD_i=\bS_{1,i}(\prod_{l=2}^L \bW_l\bS_{l,i})$ to be the $K \times K$ matrix of hidden layer evaluation for the $i^{th}$ observation. As a result, we can write $\partial_p\bPhi_{n \times K}=[(\bw_p\bD_1)^\top, \dots, (\bw_p\bD_n)^\top]^\top$, and $\partial_p\bPhi^\top\partial_p\bPhi=\sum_i \bD_i^\top\bw_p\bw_p^\top\bD_i$. Also notice that $\bPhi^+\bPhi^{+\top} = (\bPhi^\top\bPhi)_{K \times K}^{-1}$. Then simple matrix algebra yields:
\begin{align}
\psi^c_p(f) = \bw_p^\top \Big( \sum_{i=1}^n \bD_i^\top (\beta\beta^\top - (\bPhi\bPhi^\top)^{-1}) \bD_i \Big)_{K \times K} \bw_p = \bw_p^\top\bOmega \bw_p,
\label{eq:psi_compute}
\end{align}
where we have denoted $\bOmega_{K \times K}=\sum_{i=1}^n \bD_i^\top (\beta\beta^\top - (\bPhi\bPhi^\top)^{-1}) \bD_i$. It is worth noticing that the $K \times K$ ``meat" matrix $\bOmega$ does not depends on $p$ and therefore needs to be computed only once when evaluating $\psi^c_p(f)$ for all $x_p \in \{x_1, \dots, x_P\}$. The computation complexity for (\ref{eq:psi_compute}) is $O(nK^3 + PK^2)$, where $nK^3$ comes from computing the $\bOmega$ matrix for all $n$ observations, and $PK^2$ comes from computing the final $\psi^c_p(f)$ for all $P$ variables. We notice that computing (\ref{eq:psi_compute}) is much faster than the forward propagation operation a deep \gls{ReLU} network (i.e. $O(nLK^3 + nPK^2)$) which is used to generate model predictions. 

%\subsubsection*{A Parallel Extension}

For data with extremely large $n$ and $P$, it is natural to consider accelerating the computation of $\psi^c_p(f)$ by taking advantage of the modern multi-core architecture. To this end, we notice that in (\ref{eq:psi_compute}) the matrix $(\bPhi\bPhi^\top)^{-1} = (\sum_{i=1}^n \bPhi_i\bPhi_i^\top)^{-1}$ (a $O(nK^2 + K^3)$ operation) needs to be evaluated first before any other operation, creating a computation bottleneck that lead to a computation complexity of $O(nK^2/T) + O(K^3) + O(nK^3/T) + O(PK^2/T)$ given $T$ machines. Here we have written the overall time complexity as the summation of each sequential steps' complexity to stress the existence of computation bottleneck. 

To this end, we notice that a embarrassingly parallel algorithm is possible by rewriting $\psi^c_p(f)$ as:
\begin{align}
\psi^c_p(f) = tr\Big[ 
\big( \sum_{i=1}^n \bD_i\bw_p\bw_p^\top\bD_i^\top\big)
\big(\beta\beta^\top - (\bPhi\bPhi^\top)^{-1})
\Big]
=
tr\Big[ 
\bLambda_p
\big(\beta\beta^\top - (\bPhi\bPhi^\top)^{-1})
\Big],
\label{eq:psi_compute_parallel}
\end{align}
where the first matrix $\bLambda_p=\sum_{i=1}^n \bD_i\bw_p\bw_p^\top\bD_i^\top$ can be evaluated in parallel with $\bPhi\bPhi^\top$, and both operations can be distributed among multiple machines in a embarrassingly parallel fashion (see Algorithm \ref{alg:psi_compute_parallel}), thereby removing the bottleneck. The computation complexity for (\ref{eq:psi_compute_parallel}) is $O\big(nPK^2/T)+O(K^3)+O(PK^2/T\big)$, where $nPK^2$ comes from computing $\bLambda_p$ for $P$ variables across $n$ observations, $K^3$ comes from inverting the $K \times K$ matrix $\bPhi\bPhi^\top$, and $PK^2$ comes from computing $\psi^c_p(f)$ using trace operation for $P$ variables.

\begin{algorithm}[H]
\SetKwProg{PFor}{for}{ do in parallel}{end}
\SetAlgoLined
\KwIn{input weights $\{\bw_{p, K \times 1}\}_{p=1}^P$, hidden weight matrices $\{\bD_{i, K \times K}\}_{i=1}^n$.}
\KwOut{variable importance $\psi^c(f)=\{\psi^c_p(f)\}_{p=1}^P$}
 Initialize $\{\bLambda_p = \bzero_{K \times K}\}_{p=1}^P$\;
 \PFor{$i = 1, \dots, n$}{
	 \PFor{$p = 1, \dots, P$}{
		$\bLambda_{p, i} = \bLambda_{p, i-1} + \bD_i\bw_p\bw_p^\top\bD_i^\top$\;
}
	$\bPhi\bPhi^\top_i = \bPhi\bPhi^\top_{i-1} + \bPhi_i\bPhi_i^\top$\;
}
evaluate $\bM = \beta\beta^\top - (\bPhi\bPhi^\top)^{-1}$\;
\PFor{$p = 1, \dots, P$}{
	$\psi^c_p(f) = tr(\bLambda_p\bM)$
}
 \caption{Parallel Computation of Variable Importance $\psi(f)$}
 \label{alg:psi_compute_parallel}
\end{algorithm}



==> sections/proof/bvm_adaptive.tex <==
Our goal is to show:
\begin{align*}
\Pi\Big(\sqrt{n}(\psi^c_p(f) - \hat{\psi}^c_p) 
\Big| \{\bx_i, y_i\}_{i=1}^n \Big) 
\leadsto N(0, 4|| H_pf_{0} ||^2_n).
\end{align*}
First notice that by Theorem \ref{thm:bvm_fixed}, the asymptotic distribution of the marginal posterior distribution can be represented as a mixture of Gaussian:
\begin{align}
\Pi_n\Big(\sqrt{n}(\psi^c_p(f) - \hat{\psi}^c_p) \leq z \Big) 
&=
\int_\Wsc 
\Pi_n\Big(\sqrt{n}(\psi^c_p(f) - \hat{\psi}^c_{p}) \leq z | \Wsc \Big)
d\Pi_n(\Wsc) 
\nonumber\\
&= 
\int_\Wsc \Pi_n\Big(
\sqrt{n}(\psi^c_p(f) - \hat{\psi}^c_{\Wsc,p}) \leq 
z +  \sqrt{n}(\hat{\psi}^c_{p} - \hat{\psi}^c_{\Wsc,p}) 
| \Wsc \Big)d\Pi_n(\Wsc) 
\nonumber\\
&= 
\int_\Wsc \Phi\Big(
\big(z + \sqrt{n}(\hat{\psi}^c_{p} - \hat{\psi}^c_{\Wsc,p})\big)/
\sqrt{V_{\Wsc,0}} \;\big| \Wsc \Big)d\Pi_n(\Wsc) 
\label{eq:bvm_mixed_normal}
\end{align}
where the last line follows from Theorem \ref{thm:bvm_fixed}, where  $V_{\Wsc,0}=4|| H_{\Wsc,p}f_{\Wsc,0} ||^2_n$ and $\Phi$ is the standard Gaussian \gls{CDF}. 

Clearly, for \gls{BvM} to hold in the case of (\ref{eq:bvm_mixed_normal}), it is sufficient to show below two conditions \citep{castillo_bernsteinvon_2015}:
\begin{align}
|V_{\Wsc,0} - V_{0}| = o_p(1),
\quad 
\sqrt{n}|\hat{\psi}^c_{p} - \hat{\psi}^c_{\Wsc,p}| = o_p(1).
\label{eq:bvm_condition_0}
\end{align}

The first condition follows from the continuous mapping theorem for $V(H_pf_0)=2||H_pf_0||^2_n$, along with the fact that :
\begin{align*}
||H_{\Wsc,p}f_{\Wsc,0} - H_pf_0||_n 
&\leq ||(H_{\Wsc,p} - H_p)f_0||_n + 
||H_{\Wsc,p}(f_{\Wsc, 0} - f_{0})||_n
\\
&= O(||H_{\Wsc,p} - H_p||_n) + 
O(||f_{\Wsc, 0} - f_{0}||_n),\\
&= O(\frac{1}{\sqrt{n}} ||H_{\Wsc,p} - H_p||_F) + o_p(1)\\
&= O(\frac{K}{\sqrt{n}}) + o_p(1) = o_p(1),
\end{align*} 
where the first equality follows from the boundedness of $\|f_0\|_\infty$ and $\|H_{\Wsc,p}\|_\infty$ (by assumption in main article and also Proposition \ref{thm:Hp_norm}), the second equality follows from the definition of $||.||_n$ for matrix and the fact about posterior concentration of $||f - f_0||_n^2$ in the statement of Theorem \ref{thm:bvm}. The last line follows since $||\bH_p||_F=O(K)$ by Proposition (\ref{thm:Hp_norm}) and the assumption that $K=o_p(\sqrt{n})$ (Assumption (\ref{eq:tr_H_bound}) in the main article).

The second condition in (\ref{eq:bvm_condition_0}) is the important \textit{no-bias} condition which ensures that under $\Wsc \sim\Pi_n(\Wsc)$, all the conditional posterior $\psi_p^c|\Wsc$ converges toward the same target $\hat{\psi}^c_p$ \citep{castillo_bernsteinvon_2015, rousseau_frequentist_2016}. Recall that $\hat{\psi}^c_{p} = \psi_p(f_0) + 2\inner{H_pf_0}{\omega}_n + \inner{H_p\omega}{\omega}_n - E(\inner{H_p\omega}{\omega}_n)$, then the second condition can be written as:
\begin{align}
\sqrt{n}|\hat{\psi}^c_{p} - \hat{\psi}^c_{\Wsc,p} |
\leq
&
\sqrt{n}|\psi_p(f_0) - \psi_{\Wsc,p}(f_{\Wsc,0})| + 
2\sqrt{n}|
\inner{H_pf_0}{\omega}_n - 
\inner{H_{\Wsc,p}f_{\Wsc,0}}{\omega_\Wsc}_n| + 
\nonumber\\
&\sqrt{n}|\inner{H_{\Wsc,p}\omega_\Wsc}{\omega_\Wsc}_n - \inner{H_p\omega}{\omega}_n| + 
\sqrt{n}|E(\inner{H_{\Wsc,p}\omega_\Wsc}{\omega_\Wsc}_n) - E(\inner{H_p\omega}{\omega}_n)|,
\label{eq:bvm_cond2_terms}
\end{align}
where all four terms are $o_p(1)$ since they are all $O_p(K/\sqrt{n})$ and the model dimension $K$ is by assumption not too large (i.e. $K=o(n^{1/2})$). We delay the detailed arguments to the end of the proof. 

Consequently, since both conditions in (\ref{eq:bvm_condition_0}) are satisfied, the expression in (\ref{eq:bvm_mixed_normal}) converge uniquely to a normal distribution under the posterior distribution $\Pi_n(\Wsc)$, i.e.,
\begin{align}
\Pi_n\Big(\sqrt{n}(\psi^c_p(f) - \hat{\psi}^c_p) \leq z \Big) 
&= 
\int_\Wsc \Phi\Big(
\big(z + \sqrt{n}(\hat{\psi}^c_{p} - \hat{\psi}^c_{\Wsc,p})\big)/
\sqrt{V_{\Wsc,0}} \;\big| \Wsc \Big)d\Pi_n(\Wsc) 
\nonumber\\
&=
\int_\Wsc \Phi\Big(
\big(z + o_p(1)\big)/
\sqrt{V_{0} + o_p(1)} \;\big| \Wsc \Big)d\Pi_n(\Wsc) 
\nonumber\\
&= \Phi\big(z/\sqrt{V_{0}}\big), 
\qquad \mbox{where} \qquad V_0 = 4||H_0f_0||_n^2
\label{eq:bvm_mixed_normal}
\end{align}
which implies the statement of interest: 
\begin{align*}
\Pi\Big(\sqrt{n}(\psi^c_p(f) - \hat{\psi}^c_p) 
\Big| \{\bx_i, y_i\}_{i=1}^n \Big) 
\leadsto N(0, 4|| H_pf_{0} ||^2_n).
\end{align*}

\vspace{2em}
We are only left to show that all four terms in the expression (\ref{eq:bvm_cond2_terms}) are $o_p(1)$. Specifically, recall that $H_p = D_p^\top D_p$ such that $\inner{H_p a}{b}_n = \inner{D_p a}{D_p b}_n$ for any $a, b \in \Fsc$, then:

\begin{itemize}
\item \textbf{First Term}: Recall $\psi_p(f_0)=\inner{H_p f_0}{f_0}_n = ||D_p f_0||_n^2$, then the first term can be expressed as:
\begin{align*}
\sqrt{n} |\psi_p(f_0) - \psi_{\Wsc,p}(f_{\Wsc,0})|
&= 
\sqrt{n} \Big| ||D_p f_0||_n^2 - ||D_{\Wsc,p}f_{\Wsc,0}||_n^2 \Big|\\
&\leq 
\sqrt{n} \Big(
||D_p||_n^2 ||f_0||_n^2 + 
||D_{\Wsc,p}||_n^2 ||f_{\Wsc,0}||_n^2\Big) \\
&= 
\sqrt{n} \Big(O_p(||D_p||_n^2)+O_p(||D_{\Wsc,p}||_n^2) \Big) 
=
\frac{1}{\sqrt{n}} \Big(
O_p(||\bD_p||^2_F) + O_p(||\bD_{\Wsc,p}||_n^2 )\Big) \\
&= O(\frac{K}{\sqrt{n}}) = o_p(1)
\end{align*}
where on the third line, the first equality follows since $f_0$ and $f_{\Wsc,0}$ are both bounded, the second equality follows by the definition of the matrix Euclidean norm $||\bM||^2_n = \frac{1}{n}\sum_{i,j}\bM^2_{i,j}=\frac{1}{n}||\bM||^2_F$. On the last line, the first eqality follows by $||\bD_{\Wsc,p}||^2_F=tr(\bH_{\Wsc,p})=O(K)$ due to Proposition \ref{thm:Hp_norm}, and the second equality follows by Assumption $K = o_p(n^{1/2})$.

\item \textbf{Second Term}: Similarly, the second term can be expressed as:
\begin{align*}
\sqrt{n}|
\inner{H_pf_0}{\omega}_n - 
\inner{H_{\Wsc,p}f_{\Wsc,0}}{\omega_\Wsc}_n|
&= 
\sqrt{n} \big|
\inner{D_p f_0}{D_p \omega}_n - 
\inner{D_{\Wsc,p}f_{\Wsc,0}}{D_{\Wsc,p}\omega_\Wsc}_n \big|\\
&\leq 
\sqrt{n} \Big(
||D_p||_n^2 ||f_0||_n||\omega||_n + 
||D_{\Wsc,p}||_n^2 ||f_{\Wsc,0}||_n||\omega_{\Wsc}||_n \Big)\\
&=
\sqrt{n} \Big(O_p(||D_p||_n^2)+O_p(||D_{\Wsc,p}||_n^2) \Big)\\
&= O_p(\frac{K}{\sqrt{n}}) = o_p(1)
\end{align*}
where the equality on the third line follows from the fact that $f_{0, \Wsc}$ is bounded and $\omega=P_{\Fsc}\epsilon$ is a random variable with bounded variance. The rest of the equalities follow similarly as those in the First term.

\item \textbf{Third and Fourth Terms} are similar to the first term except for $f_0$ is replaced by $\omega$. As a result: 
\begin{align*}
\sqrt{n}|\inner{H_{\Wsc,p}\omega_\Wsc}{\omega_\Wsc}_n - \inner{H_p\omega}{\omega}_n| 
&=
\sqrt{n} \Big| 
||D_{\Wsc,p}\omega_\Wsc||^2_n - ||D_p\omega||^2_n 
\Big|\\
&=
\sqrt{n} \Big(O_p(||D_p||_n^2)+O_p(||D_{\Wsc,p}||_n^2) \Big)\\
&= O_p(\frac{K}{\sqrt{n}}) = o_p(1)
\\
\sqrt{n}|
E(\inner{H_{\Wsc,p}\omega_\Wsc}{\omega_\Wsc}_n) - 
E(\inner{H_p\omega}{\omega}_n)| 
&= \sqrt{n} O_p \Big( 
|\inner{H_{\Wsc,p}\omega_\Wsc}{\omega_\Wsc}_n - \inner{H_p\omega}{\omega}_n|\Big)\\
&= O_p(\frac{K}{\sqrt{n}}) = o_p(1)
\end{align*}
\end{itemize}


==> sections/proof/bvm_fixed.tex <==
Our goal is to show asymptotic normality 
$$\Pi_n\big(\sqrt{n}(\psi^c_{\Wsc,p}(f) - \hat{\psi}^c_{\Wsc,p}) | \Wsc \big) \leadsto N(0, ||\psi_{1}||_n^2).$$
First derive the expressions for $f_t, \hat{\psi}_{\Wsc,p}, V_{0, n}$ and $\Isc_{n}$. The expression for $f_t$ is:
\begin{align}
f_t &= f - 
\frac{t}{\sqrt{n}} 
\Big(
\psi_1 + \frac{1}{2} \psi_2(f - f_{0, \Wsc})\Big)  
- 
\frac{t}{2n} \psi_2(\omega_\Wsc) \nonumber \\
&= \Big( I - \frac{t}{\sqrt{n}} * H_p \Big)(f) - 
\frac{t}{\sqrt{n}} * H_p \big(f_{0, \Wsc} +  \omega_\Wsc \big).
\label{eq:ft}
\end{align}
where $I: f \rightarrow f$ is the identity operator. The expressions for $\hat{\psi}_{\Wsc,p}$ and $V_{0, n}$ are (recall $\omega_\Wsc=P_{\Fsc_\Wsc}(\epsilon)$):
\begin{align*}
\hat{\psi}_{\Wsc,p}
&= \psi_{\Wsc,p}(f_{0, \Wsc}) + 
\frac{W_n(\psi_1) }{\sqrt{n}} + 
\frac{1}{2} \frac{\inner{\omega_\Wsc}{\psi_2(\omega_\Wsc)}_n}{n}\\
&= \psi_{\Wsc,p}(f_{0, \Wsc}) + 
2 \inner{H_{\Wsc,p} f_{0, \Wsc}}{\omega_\Wsc}_n + 
\inner{H_{\Wsc,p} \omega_\Wsc}{\omega_\Wsc}_n
,
\\
V_{0, n} &= 
\Big|\Big| 
\psi_1 - \frac{1}{2} \frac{\psi_2(\omega_\Wsc)}{\sqrt{n}}
\Big|\Big|^2_n
= 
4 * \Big|\Big| 
H_{\Wsc,p}f_{0, \Wsc} + o_p(1)
\Big|\Big|^2_n,
\end{align*}
and the expression for $\Isc_{n}$ is:
\begin{align*}
\Isc_{n} = \frac{\int_{A_n} e^{l_n(f_t) - l_n(f_{0, \Wsc})} d\Pi(f | \Wsc)}
{\int_{A_n} e^{l_n(f) - l_n(f_{0, \Wsc})} d\Pi(f | \Wsc) }.
\end{align*}



It then follows from the Theorem \ref{thm:bvm_castillo} that
\begin{align}
E_n(e^{t\sqrt{n}(\psi^c_{\Wsc,p}(f) - \hat{\psi}^c_{\Wsc,p})}|A_n, \Wsc) = 
e^{o_p(1) + t^2 V_{0, n}/2} * \Isc_{n}.
\label{eq:bvm_mgf_converge}
\end{align}
Therefore to show asymptotic normality $\Pi_n\big(\sqrt{n}(\psi^c_{\Wsc,p}(f) - \hat{\psi}^c_{\Wsc,p}) | \Wsc \big) \leadsto N(0, ||\psi_1||_n^2)$, we only need to show $\Isc_{n} \rightarrow 1$ for some suitable choice of $A_n$ so that $E_n(e^{t\sqrt{n}(\psi^c_{\Wsc,p}(f) - \hat{\psi}^c_{\Wsc,p})}|A_n, \Wsc) \rightarrow e^{t^2 V_{0}/2}$. To this end, we consider the standard choice $A_n = \Big\{ f \Big| ||f - f_{0, \Wsc}||^2_n \leq M_n \epsilon_n  \Big\}$ for some sufficiently large $M_n \rightarrow \infty$ and $\epsilon_n$ the given rate of posterior convergence. 

To analyze the asymptotic behavior of $\Isc_{n}$, analogous to the Theorem 3.1 of \cite{castillo_bernsteinvon_2015}, we consider the  asymptotically equivalent term $\Isc'_{n}$:
\begin{align*}
\Isc'_{n} = \frac{\int_{f \in A_n} e^{l_n(f_t) - l_n(f_{0, \Wsc})} d\Pi(f|\Wsc)}
{\int e^{l_n(f) - l_n(f_{0, \Wsc})} d\Pi(f|\Wsc) }
\end{align*}
where the denominator $\int_{A_n}$ in $\Isc_{n}$ is replaced by $\int$. $\Isc'_{n}$ is asymptotically equivalent to $\Isc_{n}$ since $\Pi_n(A_n) = 1 + o_p(1)$. 

Notice that $\Isc'_{n}$ can be written as:
\begin{align*}
\Isc'_{n} 
&= \Jsc_n * \Ksc_n 
=
\frac{\int e^{l_n(f_t) - l_n(f_{0, \Wsc})} d\Pi(f|\Wsc)}
{\int e^{l_n(f) - l_n(f_{0, \Wsc})} d\Pi(f|\Wsc)} 
*
\frac{\int_{f \in A_n} e^{l_n(f_t) - l_n(f_{0, \Wsc})} d\Pi(f|\Wsc)}
{\int e^{l_n(f_t) - l_n(f_{0, \Wsc})} d\Pi(f|\Wsc)}
\end{align*}
where we have denoted:
\begin{align}
\Jsc_{n} &= \frac{\int e^{l_n(f_t) - l_n(f_{0, \Wsc})} d\Pi(f|\Wsc)}
{\int e^{l_n(f) - l_n(f_{0, \Wsc})} d\Pi(f|\Wsc)}, \quad
\Ksc_{n} = \frac{\int_{f \in A_n} e^{l_n(f_t) - l_n(f_{0, \Wsc})} d\Pi(f|\Wsc)}
{\int e^{l_n(f_t) - l_n(f_{0, \Wsc})} d\Pi(f|\Wsc)}.
\end{align}
Therefore in order to show $\Isc_{n} \rightarrow 1$, it is sufficient to show $\Jsc_{n} \rightarrow 1$ and $\Ksc_{n} \rightarrow 1$.

We show $\Jsc_{n} \rightarrow 1$ by first performing change of variables $f \rightarrow f_t$ on the numerator, and then analyze the asymptotic behavior of the resulting expression. To this end, notice that the conditional prior $\Pi(f|\Wsc)$ is a Gaussian process prior with kernel function $k_\Wsc(\bx, \bx')= \sum_{k=1}^K \phi_k(\bx|\Wsc)\phi_k(\bx'|\Wsc) + \sigma^2_{b_0}$, and correspondingly, the kernel matrix evaluated at $\{\bx_i, y_i\}_{i=1}^n$ is $\bK_\Wsc = \bPhi_\Wsc\bPhi_\Wsc^\top + \sigma^2_{b_0}\bI$ for $\bPhi_{n \times K}=\bX(\prod_{l=1}^L \bW_l\bS_l)$  (see Section \ref{sec:nn_mat}). Therefore given observations $\{y_i, \bx_i\}_{i=1}^n$, the conditional prior distribution for $\bdf = [f(\bx_1), \dots, f(\bx_n)]^\top \in \real^n$ is a multivariate Gaussian with covariance matrix $\bK_\Wsc$:
\begin{align*}
d\Pi(\textbf{\bdf}| \Wsc) \propto 
|\bK_{\Wsc}|^{-\frac{1}{2}} e^{-\frac{1}{2}\bdf^\top\bK_{\Wsc}^{-1}\bdf}
\end{align*}
where $|\bK_{\Wsc}| $, $\bK_{\Wsc}^{-1}$ are the determinant and inverse of $\bK_\Wsc$, respectively.  To perform change of variable, we denote $\bdf_t \in \real^n$ as $f_t$ in (\ref{eq:ft}) evaluated at $\{y_i, \bx_i\}_{i=1}^n$, we can write $\bdf_t = \bB_{t, n}\bdf - \frac{t}{\sqrt{n}}\ba_n$ such that
\begin{align*}
d\Pi(\bdf_t | \Wsc) &\propto 
|\bK_{n, \Wsc}|^{-\frac{1}{2}} 
e^{-\frac{1}{2}
(\bdf + \frac{t}{\sqrt{n}}\ba_n)^\top
\bK_{n, \Wsc}^{-1}
(\bdf + \frac{t}{\sqrt{n}}\ba_n)} \\
&= d\Pi(\bdf| \Wsc) * exp\bigg[-\frac{1}{2}
log 
\Big(\frac{|\bK_{n, \Wsc}|}{|\bK_{\Wsc}| }\Big) -
\frac{1}{2}
\bdf^\top 
\big(\bK_{n, \Wsc}^{-1}
 - \bK_{\Wsc}^{-1}\big) \bdf
+ 
\frac{t}{\sqrt{n}} \ba_n^\top\bK_{n, \Wsc}^{-1}
\bdf
-
\frac{t^2}{2n} \ba_n^\top\bK_{n, \Wsc}^{-1}
\ba_n^\top
\bigg]
\end{align*}
where 
$\bB_{t, n} = \bI - \frac{t}{\sqrt{n}} \bH_p$,
$\ba_n = \bH_p \big(\bdf_{0, \Wsc} + \omega_\Wsc \big)$, and
\begin{align*}
%\bB_{t, n} &= \bI - \frac{t}{\sqrt{n}} \bH_p,
%\quad
%\ba_n = \bH_p \big(\bdf_{0, \Wsc} + \frac{1}{\sqrt{n}} \omega_\Wsc \big), \\
\bK_{n, \Wsc} &= \bB_{t, n}\bK_{\Wsc}\bB_{t, n}
= \bK_{\Wsc} -\frac{t}{\sqrt{n}} \Big[\bK_{\Wsc}\bH_p + \bH_p\bK_{\Wsc}\bB_{t, n}\Big]
= \bK_{\Wsc} -\frac{t}{\sqrt{n}} d\bK_{\Wsc},
\end{align*}
where we have denoted $d\bK_{\Wsc} = \bK_{\Wsc}\bH_p + \bH_p\bK_{\Wsc}\bB_{t, n}$. 

Consequently, the expression of $\Jsc_{n}$ after the change of variable becomes:
\begin{align*}
\Jsc_{n} &= 
\frac
{\int e^{l_n(f_t) - l_n(f_{0, \Wsc})} * e^{-\Lsc_{t,n}} \; d\Pi(f_t|\Wsc)}
{\int e^{l_n(f) - l_n(f_{0, \Wsc})} d\Pi(f|\Wsc)},
\end{align*}
where
\begin{align}
\Lsc_{t,n} &= 
\frac{1}{2}
log 
\Big(\frac{|\bK_{n, \Wsc}|}{|\bK_{\Wsc}| }\Big) 
+
\frac{1}{2} \bdf^\top \big(\bK_{n, \Wsc}^{-1}
 - \bK_{\Wsc}^{-1}\big) \bdf
-
\frac{t}{\sqrt{n}} \ba_n^\top\bK_{n, \Wsc}^{-1}
\bdf
+
\frac{t^2}{2n} \ba_n^\top\bK_{n, \Wsc}^{-1}
\ba_n^\top.
\label{eq:L_tn}
\end{align}
Therefore in order to show $\Jsc_{n} \rightarrow 1$, it is sufficient to show that all terms in $\Lsc_{t, n}=o_p(1)$ are asymptotically vanishing toward zero as $n \rightarrow \infty$. We defer the detailed arguements to the end of this proof. If this is true, then it holds that $\Lsc_{t, n} =o_p(1)$ and 
\begin{align}
\Jsc_{n} = 
\frac
{\int e^{l_n(f_t) - l_n(f_{0, \Wsc}) + o_p(1)} \; d\Pi(f_t|\Wsc)}
{\int e^{l_n(f) - l_n(f_{0, \Wsc})} d\Pi(f|\Wsc)} \rightarrow 1.
\label{eq:Jn_converge}
\end{align}

We show $\Ksc_n \rightarrow 1$ by noticing that $\Lsc_{t, n}=o_p(1)$ implies:
\begin{align*}
\Ksc_n &=
\frac
{\int_{f \in A_n} e^{l_n(f_t) - l_n(f_{0, \Wsc})} \; d\Pi(f|\Wsc)}
{\int e^{l_n(f_t) - l_n(f_{0, \Wsc})} d\Pi(f|\Wsc)}
=
\frac
{\int_{f \in A_n} e^{l_n(f_t) - l_n(f_{0, \Wsc}) + o_p(1)} \; d\Pi(f_t|\Wsc)}
{\int e^{l_n(f_t) - l_n(f_{0, \Wsc}) + o_p(1)} d\Pi(f_t|\Wsc)}
\end{align*}
Notice that in the above expression, the event $f \in A_n$ is equivalent to $f_t \in A_{n, t}$ for:
\begin{align*}
A_{n, t} &= 
\Big\{ f_t \Big| ||f - f_0||^2_n \leq M_n \epsilon_n
\Big\}\\
&=
\Big\{ f_t \Big| ||f - f_0||^2_n \leq M_n \epsilon_n, \;
||f_t - f_0||^2_n \leq ||f_t - f||^2_n + ||f - f_0||^2_n
\Big\}\\
&\supseteq
\Big\{ f_t \Big| 
||f_t - f_0||^2_n \leq ||f_t - f||^2_n + M_n \epsilon_n
\Big\}\\
&= \Big\{ f_t \Big| 
||f_t - f_0||^2_n \leq O(n^{-1}) + M_n \epsilon_n
\Big\}\\
&= \Big\{ f_t \Big| 
||f_t - f_0||^2_n \leq M'_n \epsilon_n
\Big\}
= A'_n
\end{align*}
where on the fourth line, the equality follows since $||f_t - f||^2_n=\frac{1}{n}||\bdf_t - \bdf||^2_2 = \frac{t}{\sqrt{n}} ||\bH_p\bdf + \ba_n||^2_2/n \leq \frac{t}{\sqrt{n}}(||\bH_p||^2_2||\bdf||^2_2/n + ||\ba_n||^2_2/n)=O(n^{-\frac{1}{2}})$ since $||\bH_p||^2_2=O_p(1)$ by Proposition \ref{thm:Hp_norm}, and the facts that $||\bdf||^2_2/n=O_p(1)$ and $||\ba_n||^2_2/n=||\bH_p(\bdf_{0, \Wsc} + \omega_\Wsc)||^2/n = O_p(1)$ due to boundedness of $\bdf$, $\bdf_0$ and the fact that $\omega_\Wsc$ is a random variable with finite variance. Also, on the last line, the equality follows since $n^{-1}\lesssim \epsilon_n$, i.e. the learning rate $\epsilon_n$ is expected to be slower than $O(n^{-1})$. As a result, we see that since the set $A_n'=\Big\{ f \Big| 
||f - f_0||_n \leq M'_n \epsilon_n \Big\}$ is of the same form as $A_n$, we have that $\Pi_n(A'_n) \rightarrow 1 + o_p(1)$ due to the posterior convergence of $f$ to $f_0$. Consequently:
\begin{align}
\Ksc_n &=
\frac
{\int_{f_t \in A_{n,t}} e^{l_n(f_t) - l_n(f_{0, \Wsc}) + o_p(1)} \; d\Pi(f_t|\Wsc)}
{\int e^{l_n(f_t) - l_n(f_{0, \Wsc}) + o_p(1)} d\Pi(f_t|\Wsc)}
\geq
\frac
{\int_{f_t \in A'_{n}} e^{l_n(f_t) - l_n(f_{0, \Wsc}) + o_p(1)} \; d\Pi(f_t|\Wsc)}
{\int e^{l_n(f_t) - l_n(f_{0, \Wsc}) + o_p(1)} d\Pi(f_t|\Wsc)}
\rightarrow 1
\label{eq:Kn_converge}
\end{align}

Finally, since we have shown both $\Jsc_{n} \rightarrow 1$ and $\Ksc_{n} \rightarrow 1$, 
it then follows by Theorem \ref{thm:bvm_castillo} that the posterior distribution of $\sqrt{n}(\psi_{\Wsc,p}^c(f) - \hat{\psi}^c_\Wsc)$ converge toward a normal law with mean zero and variance $||\psi_1||_n^2 = 4 || H_{\Wsc,p}f_{0, \Wsc} ||^2_n$, i.e. we have shown the statement of the interest:
\begin{align}
\Pi\Big(\sqrt{n}(\psi^c_{\Wsc,p}(f) - \hat{\psi}^c_\Wsc) \Big| \{\bx_i, y_i\}_{i=1}^n, \Wsc \Big) \leadsto N(0, 4|| H_{\Wsc,p}f_{0, \Wsc} ||^2_n).
\label{eq:bvm_proof_conclusion}
\end{align}
\vspace{1em}

We are only left to show that $\Lsc_{t, n}=o_p(1)$, i.e. all the four terms in (\ref{eq:L_tn}) are asymptotically vanishing toward zero. We achieve this by analyzing the asymptotic behavior of the four terms one by one:
\begin{itemize}
\item First term: $log 
\Big(\frac{|\bK_{n, \Wsc}|}{|\bK_{\Wsc}| }\Big)= log |\bK_{n, \Wsc}| - log |\bK_{\Wsc}|$

Performing Taylor Expansion on $log |\bK_{n, \Wsc}|$:
%{\color{red} (make a Lemma to derive Taylor expansion).}
\footnote{For the log pseudo-determinant function $f(\bX) = log |\bX|$, we can compute its gradient function as $\nabla_{\bX} f(\bX) = \bX^+$ Hessian 
%\citep{holbrook_differentiating_2018}, and \href{https://www.quora.com/What-is-the-derivative-of-inverse-matrix}{Hessian} 
$H_{\bX} f(\bX) = \bX^+ \otimes \bX^+$.}
\footnote{The second-order term in Taylor expansion is $vec(d\bK_{\Wsc})^\top(\bK_{\Wsc}^{-1} \otimes \bK_{\Wsc}^{-1})vec(d\bK_{\Wsc})$. Using property of Kronecker product $(\bC^\top \otimes \bA)vec(\bB) = vec(\bA\bB\bC)$, the second-order term can also be written as 
$vec(d\bK_{\Wsc})^\top vec(\bK_{\Wsc}^{-1} d\bK_{\Wsc} \bK_{\Wsc}^{-1}) 
= tr(d\bK_{\Wsc}\bK_{\Wsc}^{-1} d\bK_{\Wsc} \bK_{\Wsc}^{-1}) 
= tr((\bK_{\Wsc}^{-1} d\bK_{\Wsc})^2)
\leq tr(\bK_{\Wsc}^{-1} d\bK_{\Wsc})^2
$, 
where the last inequality follows from the fact that $\bK_{\Wsc}^{-1} d\bK_{\Wsc}$ is  positive semidefinite.
}
\begin{align}
log |\bK_{n, \Wsc}| 
&= log \Big|\bK_{\Wsc} -\frac{t}{\sqrt{n}}d\bK_{\Wsc}\Big|
\nonumber \\
&= log |\bK_{\Wsc}| - \frac{t}{\sqrt{n}} tr(\bK_{\Wsc}^{-1} d\bK_{\Wsc}) + \frac{t^2}{n} O_p\big(tr(\bK_{\Wsc}^{-1} d\bK_{\Wsc})^2 \big) .
\label{eq:log_det_K}
\end{align}
where
\begin{align}
\frac{t}{\sqrt{n}} tr(\bK_{\Wsc}^{-1}d\bK_{\Wsc}) 
&= 
\frac{t}{\sqrt{n}} tr\Big(\bK_{\Wsc}^{-1}(\bK_{\Wsc}\bH_{\Wsc,p} + \bH_{\Wsc,p}\bK_{\Wsc} -\frac{t}{\sqrt{n}} \bH_{\Wsc,p}\bK_{\Wsc}\bH_{\Wsc,p})\Big)
\nonumber\\
& = \frac{2t}{\sqrt{n}} tr(\bH_{\Wsc,p}) - \frac{t^2}{n} tr(\bK_{\Wsc}^{-1}\bH_{\Wsc,p}\bK_{\Wsc}\bH_{\Wsc,p}) 
\nonumber \\
& \leq \frac{2t}{\sqrt{n}} tr(\bH_{\Wsc,p})
\nonumber \\
& = \frac{t}{\sqrt{n}} O_p(K).
\label{eq:Kinv_dK}
\end{align}
In the above expression, the inequality follows from the fact that $\bK_{\Wsc}^{-1}\bH_{\Wsc,p}\bK_{\Wsc}\bH_{\Wsc,p}$ is positive semi-definite, and the last line follows from Proposition \ref{thm:Hp_norm}, i.e., $tr(\bH_{\Wsc,p}) = O_p(K)$.

By combing (\ref{eq:log_det_K}) and (\ref{eq:Kinv_dK}):
\begin{align}
log |\bK_{n, \Wsc}| - log |\bK_{\Wsc}| 
& = - \frac{t}{\sqrt{n}} tr(\bK_{\Wsc}^{-1} d\bK_{\Wsc}) + \frac{t^2}{n} O_p\big(tr(\bK_{\Wsc}^{-1} d\bK_{\Wsc})^2 \big) 
= t * O_p(\frac{K}{\sqrt{n}}) = o_p(1).
\label{eq:term_1_bound}
\end{align}
where recall $O_p(\frac{K}{\sqrt{n}}) = o_p(1)$ since $K=o_p(n^{1/2})$.

\item Second term: $\bdf^\top 
\big(\bK_{n, \Wsc}^{-1}
 - \bK_{\Wsc}^{-1}\big) \bdf
$

Bound this term using the Cauchy-Schwarz inequality $\bdf^\top 
\big(\bK_{n, \Wsc}^{-1}
 - \bK_{\Wsc}^{-1}\big) \bdf 
\leq ||\bK_{n, \Wsc}^{-1}
  - \bK_{\Wsc}^{-1}||_\infty||\bdf||_\infty^2$, where recall $||.||_2$ denotes the matrix 2-norm, i.e., the largest singular value. Notice that by applying the inversion formula
 %\href{https://math.stackexchange.com/questions/17776/inverse-of-the-sum-of-matrices}{inversion formula} 
  $(\bA + \bB)^{-1} = \bA^{-1} - \bA^{-1} \bB (\bA + \bB)^{-1}$ \citep{henderson_deriving_1981}, we have $\bK_{n, \Wsc}^{-1}
  - \bK_{\Wsc}^{-1} = \frac{t}{\sqrt{n}} (\bK_{\Wsc}^{-1}d\bK_{\Wsc})\bK_{n, \Wsc}^{-1}
$, and further manipulation reveals that:
\begin{align*}
\bK_{\Wsc}^{-1}d\bK_{\Wsc}\bK_{n, \Wsc}^{-1}
 &= 
\bK_{\Wsc}^{-1} (\bK_{\Wsc}\bH_{\Wsc,p} + \bH_{\Wsc,p}\bK_{\Wsc}\bB_{t, n}) (\bB_{t, n}^+\bK_{\Wsc}^{-1}\bB_{t, n}^+)
= 
\bH_{\Wsc,p}\bB_{t, n}^+\bK_{\Wsc}^{-1}\bB_{t, n}^+ + \bK_{\Wsc}^{-1}\bH_{\Wsc,p}\bB_{t, n}^+
%\\&= (\bH_{\Wsc,p}^+ - \frac{t}{\sqrt{n}}\bI)^+\bK_{\Wsc}^{-1}(\bH_{\Wsc,p}^+ - \frac{t}{\sqrt{n}}\bI)^+\bH_{\Wsc,p}^+ + \bK_{\Wsc}^{-1}(\bH_{\Wsc,p}^+ - \frac{t}{\sqrt{n}}\bI)^+
\end{align*}
Then, by triangular inequality, we can bound $||\bK_{n, \Wsc}^{-1}||_\infty$ as:
\begin{align}
||\bK_{n, \Wsc}^{-1}
  - \bK_{\Wsc}^{-1}||_\infty
&= \frac{t}{\sqrt{n}} ||\bK_{\Wsc}^{-1}d\bK_{\Wsc}\bK_{n, \Wsc}^{-1}
||_\infty
\nonumber\\
&\leq \frac{t}{\sqrt{n}} \Big(
||\bH_{\Wsc,p}\bB_{t, n}^+\bK_{\Wsc}^{-1}\bB_{t, n}^+||_\infty + ||\bK_{\Wsc}^{-1}\bH_{\Wsc,p}\bB_{t, n}^+||_\infty\Big)
\nonumber\\
&= \frac{t}{\sqrt{n}} \Big(
||\bB_{t, n}^+\bH_{\Wsc,p}\bK_{\Wsc}^{-1}\bB_{t, n}^+||_\infty + ||\bK_{\Wsc}^{-1}\bH_{\Wsc,p}\bB_{t, n}^+||_\infty\Big)
\nonumber\\
&\leq \frac{t}{\sqrt{n}} \Big(
||\bH_{\Wsc,p}\bK_{\Wsc}^{-1}||_\infty||\bB_{t, n}^+||^2_\infty + ||\bK_{\Wsc}^{-1}\bH_{\Wsc,p}||_\infty||\bB_{t, n}^+||_\infty\Big)
\nonumber\\
&= \frac{t}{\sqrt{n}} \Big(
||\bH_{\Wsc,p}\bK_{\Wsc}^{-1}||_\infty + ||\bK_{\Wsc}^{-1}\bH_{\Wsc,p}||_\infty\Big)
= \frac{2t}{\sqrt{n}} ||\bK_{\Wsc}^{-1}\bH_{\Wsc,p}||_\infty
\nonumber\\
&\leq \frac{2t}{\sqrt{n}} ||\bK_{\Wsc}^{-1}||_\infty*||\bH_{\Wsc,p}||_\infty
=
t*O_p(n^{-1/2}),
\label{eq:K_inv_diff}
\end{align}
where the second equality follows since $\bH_{\Wsc,p}\bB_{t, n}^+ =\bB_{t, n}^+\bH_{\Wsc,p}$ due to the fact that $\bB_{t, n}^+ = \bH_{\Wsc,p}^+(\bH_{\Wsc,p}^+ - \frac{t}{\sqrt{n}}\bI)^+= (\bH_{\Wsc,p}^+ - \frac{t}{\sqrt{n}}\bI)^+\bH_{\Wsc,p}^+$. The third equality follows since $||\bB^{+}_{t,n}||_\infty \leq ||\bB^{+}_{t,n}||_2 = ||(\bI - \frac{t}{\sqrt{n}}\bH_{\Wsc,p})^+||_2 = 1$ due to the fact that $\bH_{\Wsc,p}$ is not full-column rank, and the last line follows by the facts that $||\bK_{\Wsc}^{-1}||_\infty \leq ||\bK_{\Wsc}^{-1}||_2 = O_p(1)$ due to $\bK_\Wsc = \bPhi_\Wsc\bPhi_\Wsc^\top + \sigma^2_{b_0}\bI$ and  $||\bH_{\Wsc,p}||_\infty \leq ||\bH_{\Wsc,p}||_2 = o_p(1)$ due to Proposition \ref{thm:Hp_norm}.

Finally, we know $||\bdf||^2_\infty = C_f^2 = o_p(1)$ due to  assumption that $||f_0||_\infty < C_f$ . As a result, the term $\bdf^\top \big(\bK_{n, \Wsc}^{-1}
 - \bK_{\Wsc}^{-1}\big) \bdf$ can be bounded as:
\begin{align}
\bdf^\top 
\big(\bK_{n, \Wsc}^{-1}
 - \bK_{\Wsc}^{-1}\big) \bdf 
&\leq 
||\bK_{n, \Wsc}^{-1}
 - \bK_{\Wsc}^{-1}||_\infty ||\bdf||_\infty^2 
= t * O_p(n^{-\frac{1}{2}}) = o_p(1).
\label{eq:term_2_bound}
\end{align}

\item Third and fourth term: $\frac{t}{\sqrt{n}} \ba_n^\top\bK_{n, \Wsc}^{-1}
\bdf$ and $\frac{t^2}{2n} \ba_n^\top\bK_{n, \Wsc}^{-1}
\ba_n^\top$.

First notice that:
\begin{align*}
||\bK_{n, \Wsc}^{-1}
||_\infty 
&= ||\bB^{+}_{t,n}\bK_{\Wsc}^{-1}\bB^{+}_{t,n}||_\infty 
\leq  ||\bK_{\Wsc}^{-1}||_\infty ||\bB^{+}_{t,n}||^2_\infty 
= ||\bK_{\Wsc}^{-1}||_\infty = O_p(1)
\end{align*}
where the second equality follows since $||\bB^{+}_{t,n}||_\infty \leq ||\bB^{+}_{t,n}||_2  = ||(\bI - \frac{t}{\sqrt{n}}\bH_{\Wsc,p})^+||_2 = 1$ due to the fact that $\bH_{\Wsc,p}$ is not full-column rank. The final equality follows from the fact that $||\bK_{\Wsc}^{-1}||_\infty \leq |\bK_{\Wsc}^{-1}||_2 = \sigma^{-2}_{b_0} = O_p(1)$ due to $\bK_\Wsc = \bPhi_\Wsc\bPhi_\Wsc^\top + \sigma^2_{b_0}\bI$.

Also notice that 
\begin{align*}
||\ba_n||_\infty 
= ||\bH_{\Wsc,p}(\bdf_{0, \Wsc} + \omega_\Wsc)||_\infty 
&\leq ||\bH_{\Wsc,p}||_\infty ||\bdf_{0, \Wsc}||_\infty + 
||\omega_\Wsc||_\infty\\
&\leq ||\bH_{\Wsc,p}||_2 ||\bdf_{0, \Wsc}||_\infty + 
||\omega_\Wsc||_2
= O_p(1)
\end{align*}
since $||\omega_\Wsc||_2 = O_p(1)$, $||\bdf_{0, \Wsc}||_\infty = C_f = O_p(1)$ and $||\bH_{\Wsc,p}||_2 = O_p(1)$ by Proposition \ref{thm:Hp_norm}. Also
\begin{align*}
||\bdf||_\infty 
= ||\bX (\prod_{l=1}^L \bW_l\bS_l)\bbeta||_{\infty}
&\leq ||\bX||_{\infty} * \prod_{l=1}^L (||\bW_l||_{\infty} ||\bS_l||_{\infty}) * ||\bbeta||_{\infty} = O_p(1)
\end{align*}
since  $||\bW_l||_{\infty} \leq B \leq 1$, $||\bbeta||_{\infty} \leq B \leq 1$, and the fact that elements in $\bX$ and $\bS_l$ are bounded between $(0, 1)$.

Therefore we can bound $\frac{t}{\sqrt{n}} \ba_n^\top\bK_{n, \Wsc}^{-1}
\bdf$ as:
\begin{align}
\frac{t}{\sqrt{n}} \ba_n^\top\bK_{n, \Wsc}^{-1}
\bdf 
&\leq \frac{t}{\sqrt{n}} ||\ba_n||_\infty ||\bK_{n, \Wsc}^{-1}
||_\infty||\bdf||_\infty
\leq t * O_p(n^{-\frac{1}{2}})=o_p(1).
\label{eq:term_3_bound}
\end{align}

Similarly, we can bound the fourth term $\frac{t^2}{2n} \ba_n^\top\bK_{n, \Wsc}^{-1}
\ba_n^\top$ as:
\begin{align}
\frac{t^2}{2n} \ba_n^\top\bK_{n, \Wsc}^{-1}
\ba_n^\top
&\leq \frac{t^2}{2n} ||\ba_n||^2_\infty  ||\bK_{n, \Wsc}^{-1}
||_\infty 
\leq t^2 * O_p(n^{-1})=o_p(1).
\label{eq:term_4_bound}
\end{align}

\end{itemize}

Consequently, by combining the asymptotic bounds for the four terms (\ref{eq:term_1_bound}), (\ref{eq:term_2_bound}), (\ref{eq:term_3_bound}) and (\ref{eq:term_4_bound}), we have that 
\begin{align*}
\Jsc_{n} 
&= 
\frac{
\int e^{l_n(f_t) - l_n(f_{0, \Wsc})} * e^{-\Lsc_{t,n}} \; d\Pi(f_t | \Wsc)}
{\int e^{l_n(f) - l_n(f_{0, \Wsc})} d\Pi(f |\Wsc)}
=
e^{-\frac{t}{\sqrt{n}} o_p(K)}
\rightarrow 1,
\end{align*}
where the last equality follows since $K/\sqrt{n} = o_p(1)$ due to Assumption  (\ref{eq:tr_H_bound}). 



==> sections/proof/bvm_mvn_adaptive.tex <==
Our goal is to show:
\begin{align}
\Pi\Big(\sqrt{n}(\psi^c(f) - \hat{\psi}^c) 
\Big| \{\bx_i, y_i\}_{i=1}^n \Big) 
\leadsto N(0, V_0).
\label{eq:bvm_mvn_statement}
\end{align}
We show the convergence of above multivariate normal distribution by involing the Cram\'{e}r-Wold device, i.e. we show that for all $t \in \real^P$:
\begin{align*}
\Pi\Big(\sqrt{n} \, (t^\top\psi^c(f) - t^\top\hat{\psi}^c) 
\Big| \{\bx_i, y_i\}_{i=1}^n \Big) 
\leadsto N(0, t^\top V_0 t).
\end{align*}

Similar to the scalar case, the asymptotic distribution of the marginal posterior distribution can be represented as a mixture of Gaussian:
\begin{align}
\Pi_n\Big(\sqrt{n}(t^\top\psi^c(f) - t^\top\hat{\psi}^c) \leq z \Big) 
&=
\int_\Wsc 
\Pi_n\Big(t^\top\sqrt{n}(\psi^c(f) - t^\top\hat{\psi}^c_{p}) \leq z | \Wsc \Big)
d\Pi_n(\Wsc) 
\nonumber\\
&= 
\int_\Wsc \Pi_n\Big(
\sqrt{n}(t^\top\psi^c(f) - t^\top\hat{\psi}^c_{\Wsc,p}) \leq 
z +  \sqrt{n}(t^\top\hat{\psi}^c_{p} - t^\top\hat{\psi}^c_{\Wsc,p}) 
| \Wsc \Big)d\Pi_n(\Wsc) 
\nonumber\\
&= 
\int_\Wsc \Phi\Big(
\big(z + \sqrt{n}(t^\top\hat{\psi}^c_{p} - t^\top\hat{\psi}^c_{\Wsc,p})\big)/
\sqrt{t^\top V_{\Wsc,0} t} \;\big| \Wsc \Big)d\Pi_n(\Wsc) 
\label{eq:bvm_mvn_mixed_normal}
\end{align}
where the last line follows from Theorem \ref{thm:bvm_mvn_fixed}, where  $(V_{0,\Wsc})_{p_1, p_2} =  4\inner{H_{\Wsc,p_1}f_{0,\Wsc}}{H_{\Wsc,p_2}f_{0,\Wsc}}_n$ and $\Phi$ is the standard Gaussian \gls{CDF}. 

Therefore it is sufficient to show below two conditions \citep{castillo_bernsteinvon_2015}:
\begin{align}
t^\top(V_{\Wsc,0} - V_{0}) t = o_p(1),
\quad 
\sqrt{n}|t^\top\hat{\psi}^c - t^\top\hat{\psi}^c_{\Wsc}| = o_p(1).
\label{eq:bvm_condition_1}
\end{align}
However, both conditions follows from the coordinate-wise convergence $\sqrt{n}|\hat{\psi}^c_{p} - \hat{\psi}^c_{\Wsc,p}| = o_p(1)$ and $||H_{\Wsc,p}f_{\Wsc,0} - H_pf_0||_n = o_p(1)$, which were established in the proof for Theorem \ref{thm:bvm}.

Consequently, the expression in (\ref{eq:bvm_mvn_mixed_normal}) converge uniquely to a normal distribution under the posterior distribution $\Pi_n(\Wsc)$, i.e.,
\begin{align*}
\Pi_n\Big(\sqrt{n}(t^\top\psi^c(f) - t^\top\hat{\psi}^c) \leq z \Big) 
&= 
\int_\Wsc \Phi\Big(
\big(z + \sqrt{n}(t^\top\hat{\psi}^c_{p} - t^\top\hat{\psi}^c_{\Wsc,p})\big)/
\sqrt{t^\top V_{\Wsc,0} t} \;\big| \Wsc \Big)d\Pi_n(\Wsc) 
\nonumber\\
&=
\int_\Wsc \Phi\Big(
\big(z + o_p(1)\big)/
\sqrt{t^\top V_{0} t + o_p(1)} \;\big| \Wsc \Big)d\Pi_n(\Wsc) 
\nonumber\\
&= \Phi\big(z/\sqrt{t^\top V_{0} t}\big), 
\qquad \mbox{where} \qquad (V_{0})_{p_1, p_2} =  4\inner{H_{p_1}f_{0}}{H_{p_2}f_{0}}_n
%\label{eq:bvm_mixed_normal_2}
\end{align*}
which implies the statement of interest (\ref{eq:bvm_mvn_statement}).



==> sections/proof/bvm_mvn_fixed.tex <==
Our goal is to show the asymptotic normality 
$$\Pi_n\big(\sqrt{n}(\psi^c_\Wsc(f) - \hat{\psi}^c_\Wsc) \big| \Wsc \big) \leadsto MVN(0, V_{0,\Wsc}).$$
First derive the expressions for $f_t, \hat{\psi}_\Wsc, V_{0, n}$ and $\Isc_{n}$. For $t = [t_1, \dots, t_P] \in \real^P$, the expression for $f_t$ is:
\begin{align}
f_t &= f - 
\frac{t^\top}{\sqrt{n}} 
\Big(
\psi_1 + \frac{1}{2} \psi_2(f - f_{0,\Wsc})\Big)  
- 
\frac{t^\top}{2n} \psi_2(\omega_\Wsc) \nonumber \\
&= \Big( I - \frac{t^\top}{\sqrt{n}} * H_\Wsc \Big)(f) - 
\frac{t^\top}{\sqrt{n}} * H_\Wsc \big(f_{0,\Wsc} + \omega_\Wsc \big).
\label{eq:mvn_ft}
\end{align}
The expressions for $\hat{\psi}_\Wsc$ and $t^\top V_{0, n} t$ are:
\begin{align*}
\hat{\psi}_\Wsc 
&= \hat{\psi}(f_{0,\Wsc}) + 
\frac{W_n(\psi_1) }{\sqrt{n}} + 
\frac{1}{2} \frac{\inner{\omega_\Wsc}{\psi_2(\omega_\Wsc)}_n}{n}\\
&= \hat{\psi}(f_{0,\Wsc}) + 2 \inner{H_\Wsc f_{0,\Wsc}}{\omega_\Wsc}_n + \inner{H_\Wsc \omega_\Wsc}{\omega_\Wsc}_n
,
\\
t^\top V_{0, n} t &= 
\Big|\Big| 
t^\top(\psi_1 - \frac{1}{2} \frac{\psi_2(\omega_\Wsc)}{\sqrt{n}})
\Big|\Big|^2_n
= 
4 * \Big|\Big| 
t^\top H_\Wsc f_{0,\Wsc} + o_p(1)
\Big|\Big|^2_n,
\end{align*}
and the expression for $\Isc_{n}$ is:
\begin{align*}
\Isc_{n} = \frac{\int_{A_n} e^{l_n(f_t) - l_n(f_{0,\Wsc})} d\Pi(f| \Wsc)}
{\int_{A_n} e^{l_n(f) - l_n(f_{0,\Wsc})} d\Pi(f|\Wsc) }.
\end{align*}
It then follows from the Theorem \ref{thm:bvm_castillo} that
$$E_n(e^{t^\top\sqrt{n}(\psi^c_\Wsc(f) - \hat{\psi}^c_\Wsc )}|A_n, \Wsc) = 
e^{o_p(1) + t^\top V_{0, n} t/2} * \Isc_{n}.$$ 
Therefore to show asymptotic normality, we only need to show $\Isc_{n} \rightarrow 1$ for some suitable choice of $A_n$ so that $E_n(e^{t^\top \sqrt{n}(\hat{\psi}^c_p(f) - \hat{\psi}^c)}|A_n, \Wsc) \rightarrow e^{t^\top V_{0, \Wsc} t/2}$. 

To this end, we consider the standard choice $A_n = \Big\{ f \Big| ||f - f_{0,\Wsc}||_n \leq M_n \epsilon_n  \Big\}$ for some sufficiently large $M_n \rightarrow \infty$ and $\epsilon_n$ the given rate of posterior convergence. Similar to the proof for Theorem \ref{thm:bvm_castillo}, it is sufficient to show the terms $\Jsc_{n} \rightarrow 1$ and $\Ksc_{n} \rightarrow 1$, where
\begin{align*}
\Jsc_{n} = \frac{\int e^{l_n(f_t) - l_n(f_{0,\Wsc})} d\Pi(f| \Wsc)}
{\int e^{l_n(f) - l_n(f_{0,\Wsc})} d\Pi(f|\Wsc)}, \quad
\Ksc_{n} = \frac{\int_{f \in A_n} e^{l_n(f_t) - l_n(f_{0, \Wsc})} d\Pi(f|\Wsc)}
{\int e^{l_n(f_t) - l_n(f_{0, \Wsc})} d\Pi(f|\Wsc)}.
\end{align*}

The argument for $\Ksc_n \rightarrow 1$ is essentially the same as those in the proof for Theorem \ref{thm:bvm_fixed} (i.e.,  (\ref{eq:Kn_converge})). We show $\Jsc_{n} \rightarrow 1$ by performing change of variables $f \rightarrow f_t$ on the numerator, and then analyze the asymptotic behavior of the resulting expression. Similar to the proof for Theorem \ref{thm:bvm_castillo}, by noticing the conditional prior $\Pi(f|\Wsc)$ is a Gaussian process prior with kernel matrix $\bK_\Wsc = \bPhi_\Wsc\bPhi_\Wsc^\top + \sigma^2_{b_0}\bI$ for $\bPhi_{n \times K}=\bX(\prod_{l=1}^L \bW_l\bS_l)$, we see that given observations $\{y_i, \bx_i\}_{i=1}^n$, the conditional prior distribution for $\bdf = [f(\bx_1), \dots, f(\bx_n)]^\top \in \real^n$ is a multivariate Gaussian with covariance matrix $\bK_\Wsc$:
\begin{align*}
d\Pi(\textbf{\bdf}| \Wsc) \propto 
|\bK_{\Wsc}| ^{-\frac{1}{2}} e^{-\frac{1}{2}\bdf^\top\bK_{\Wsc}^{-1}\bdf}.
\end{align*}
To perform change of variable, we denote $\bdf_t \in \real^n$ as $f_t$ in (\ref{eq:mvn_ft}) evaluated at $\{y_i, \bx_i\}_{i=1}^n$, we can write $\bdf_t = \bB_{t, n}\bdf - \frac{1}{\sqrt{n}}\ba_n$ such that
\begin{align*}
d\Pi(\bdf_t | \Wsc) &\propto 
|\bK_{n, \Wsc}|^{-\frac{1}{2}} 
e^{-\frac{1}{2}
(\bdf + \frac{1}{\sqrt{n}}\ba_n)^\top
\bK_{n, \Wsc}^{-1}
(\bdf + \frac{1}{\sqrt{n}}\ba_n)} \\
&= d\Pi(\bdf| \Wsc) * exp\bigg[-\frac{1}{2}
log 
\Big(\frac{|\bK_{n, \Wsc}|}{|\bK_{\Wsc}| }\Big) -
\frac{1}{2}
\bdf^\top 
\big(\bK_{n, \Wsc}^{-1} - \bK_{\Wsc}^{-1}\big) \bdf
+ 
\frac{1}{\sqrt{n}} \ba_n^\top\bK_{n, \Wsc}^{-1}\bdf
-
\frac{1}{2n} \ba_n^\top\bK_{n, \Wsc}^{-1}\ba_n^\top
\bigg]
\end{align*}
where 
$\bB_{t, n} = \bI - \frac{1}{\sqrt{n}} \bH_t$,
$\ba_n = \bH_t \big(\bdf_{0,\Wsc} + \omega_\Wsc \big)$ for $\bH_t = \sum_{p=1}^P t_p \bH_p$, and
\begin{align*}
%\bB_{t, n} &= \bI - \frac{1}{\sqrt{n}} \bH_t,
%\quad
%\ba_n = \bH_t \big(\bdf_{0,\Wsc} + \frac{1}{\sqrt{n}} \omega_\Wsc \big), \\
\bK_{n, \Wsc} &= \bB_{t, n}\bK_{\Wsc}\bB_{t, n}
= \bK_{\Wsc} -\frac{1}{\sqrt{n}} \Big[\bK_{\Wsc}\bH_t + \bH_t\bK_{\Wsc}\bB_{t, n}\Big]
= \bK_{\Wsc} -\frac{1}{\sqrt{n}} d\bK_{\Wsc},
\end{align*}
where we have denoted $d\bK_{\Wsc} = \bK_{\Wsc}\bH_t + \bH_t\bK_{\Wsc}\bB_{t, n}$. 

Consequently, the expression of $\Jsc_{n}$ after the change of variable becomes:
\begin{align*}
\Jsc_{n} &= 
\frac
{\int e^{l_n(f_t) - l_n(f_{0,\Wsc})} * e^{-\Lsc_{t,n}} \; d\Pi(f_t| \Wsc)}
{\int e^{l_n(f) - l_n(f_{0,\Wsc})} d\Pi(f|\Wsc)},
\end{align*}
where
\begin{align}
\Lsc_{t,n} &= 
\frac{1}{2}
log 
\Big(\frac{|\bK_{n, \Wsc}|}{|\bK_{\Wsc}| }\Big) 
+
\frac{1}{2} \bdf^\top \big(\bK_{n, \Wsc}^{-1} - \bK_{\Wsc}^{-1}\big) \bdf
-
\frac{1}{\sqrt{n}} \ba_n^\top\bK_{n, \Wsc}^{-1}\bdf
+
\frac{t^2}{2n} \ba_n^\top\bK_{n, \Wsc}^{-1}\ba_n^\top.
\label{eq:L_tn_mvn}
\end{align}
Therefore in order to show $\Jsc_{n} \rightarrow 1$, it is sufficient to show that all terms in $\Lsc_{t, n}$ are asymptotically vanishing toward zero as $n \rightarrow \infty$. Now only left to show that all the four terms in (\ref{eq:L_tn_mvn}) are asymptotically vanishing toward zero. However, notice that the only difference between (\ref{eq:L_tn_mvn}) and its counterpart (\ref{eq:L_tn}) in the proof of Theorem \ref{thm:bvm_fixed} is that $\bH_p$ is replaced by $\bH_t=\sum_{p=1}^P t_p\bH_p$. Furthermore, for fixed $t$, the asymptotic behavior of $\bH_p$ and $\bH_t$ are similar in the sense that $tr(\bH_t)=O_p(K)$ and $||\bH_t||_2=O_p(1)$ since $P=O(1)$. Therefore we can follow exactly the same arguments as those in the proof for Theorem \ref{thm:bvm_fixed} to show all the four terms asymptotically vanishing towards zero. Consequently, we have that 
$
\Jsc_{n} 
= 
\frac{
\int e^{l_n(f_t) - l_n(f_{0,\Wsc}) + o_p(1)} \; d\Pi(f_t| \Wsc)}
{\int e^{l_n(f) - l_n(f_{0,\Wsc})} d\Pi(f|\Wsc)} 
\rightarrow 1.
$.

It then follows by the semi-parametric \gls{BvM} theorem (Theorem \ref{thm:bvm_castillo}) that the posterior distribution of $\sqrt{n}(\psi^c_\Wsc(f) - \hat{\psi}^c_\Wsc)$ converge toward a normal law with mean zero and variance $V_0$, i.e. 
\begin{align}
\Pi\Big(\sqrt{n}(\psi^c_\Wsc(f) - \hat{\psi}^c_\Wsc) \Big| \{\bx_i, y_i\}_{i=1}^n \Big) \leadsto N(0, V_0),
\label{eq:bvm_proof_conclusion}
\end{align}
where $V_0$ is the $P \times P$ matrix that takes value $t^\top V_{0, n} t = 4 * || t^\top H_\Wsc f_{0,\Wsc} ||^2_n$ for any $t \in \real^P$. Specifically, the matrix $V_0$ whose $(p_1, p_2)^{th}$ entry defined as $4 \inner{H_{p_1}f_{0,\Wsc}}{H_{p_2}f_{0,\Wsc}}_n $ will satisfy this choice.


==> sections/proof/f_post_converg.tex <==
 We show posterior consistency by invoking Theorem 1 of \cite{ghosal_convergence_2000}. As argued in \citep{rockova_posterior_2018} (Proof for Theorem 6.1), it is sufficient to show below two conditions about the prior distribution:
\begin{align}
log N(\epsilon_n, \Fsc, ||.||_\infty) \leq C n \epsilon_n
\label{eq:entropy_cond}
\\
\Pi \Big(||f - f_0||^2_\infty \leq \epsilon_n \Big) \geq e^{-C n \epsilon_n}
\label{eq:prior_cond}
\end{align}
where $C > 1$ is an universal constant. The first condition (\ref{eq:entropy_cond}) ensures the model size, which is measured by the covering number of $\Fsc$ (i.e., the minimal number of $||.||_\infty$-balls with radius $\delta$ that covers $\Fsc$) is not too large. The second condition (\ref{eq:prior_cond}) ensures the model 's  prior distribution places sufficient prior mass around the target function $f_0$. For the rest of this proof, we show the statement of interest by showing these two conditions.

\begin{itemize}
\item \textbf{Entropy Condition}: $log N(\epsilon_n, \Fsc, ||.||_n) \leq n \epsilon_n$

We show this condition by invoking the classic result on the covering number of neural network approximation spaces (Lemma \ref{thm:cover_number}) \citep{anthony_neural_2009} . Specifically, by setting $\delta = \epsilon_n$ in Lemma 3, we have 
\begin{align*}
log N(\epsilon_n, \Fsc, ||.||_\infty) 
&\leq S \, log(\epsilon_n^{-1} L (K+1)^{2L} )\\
&\lesssim S \, log(\epsilon_n^{-1}) + S \, L \, log(K)\\
&\lesssim N \, log(N) \, log(\frac{n}{N log(N)^3}) + N log(N)^3\\
&\lesssim N \, log(N) \, (log(n) + log(N)^2)\\
&\lesssim N \, log(N)^3 = n \epsilon_n
\end{align*}
where the last line follows from the assumption that $log (N) \geq \sqrt{log(n)}$ and the definition of $\epsilon_n$.

\item \textbf{Prior Mass Condition}: $\Pi \Big(||f - f_0||_n \leq \epsilon_n \Big) \geq e^{-C n \epsilon_n}$.

We show this using the classic concentration inequality for the centered Gaussian measure $\Pi$ (Lemma \ref{thm:shift_ball_ineq}). First notice that as argued in the proof of Theorem 6.1 of \cite{rockova_posterior_2018}, by the proof of Lemma 5 of \cite{schmidt-hieber_nonparametric_2017}:
\begin{align*}
\Big\{ f \Big| ||f - f_0||^2_\infty \leq \epsilon_n \Big\} \subset 
\Big\{ \Wsc \Big| ||\Wsc - \Wsc_0||^2_\infty \leq \frac{\epsilon_n}{(V(L+1))^2} \Big\}
\end{align*}
where $V = O\big( P * K^{L} \big)$. Therefore
\begin{align*}
\Pi \Big(||f - f_0||^2_\infty \leq \epsilon_n \Big) 
&\geq 
\Pi \Big(||\Wsc - \Wsc_0||^2_\infty \leq \frac{\epsilon_n}{(V(L+1))^2} \Big)\\
&\geq 
exp \Big(-\frac{||\Wsc_0||_\Pi^2}{2}\Big)
\Pi \Big(||\Wsc||^2_\infty < \frac{\epsilon_n}{(V(L+1))^2} \Big)\\
& \geq 
exp \Big(-\frac{||\Wsc_0||_\Pi^2}{2}\Big)
exp \Big(-\frac{\epsilon_n}{(V(L+1))^2}\Big)\\
& \geq exp(-Cn \epsilon_n)
\end{align*}
for some $C>1$. In the above expression, the second inequality follows from Lemma \ref{thm:shift_ball_ineq}, and the third inequality follows from the Borell's inequality \citep{van_der_vaart_reproducing_2008}. 
\end{itemize}


==> sections/proof/post_convergence.tex <==
Denote $A_n = \{f : ||f - f_0||^2_n > M_n \epsilon_n \}$ and $B_n = \{f : |\psi_p(f) - \Psi_p(f_0)| > M_n \epsilon_n \}$, then showing the statement in Theorem \ref{thm:post_convergence} is equivalent to showing $\Pi_n(B_n) \rightarrow 0$.

Specifically, we assume below three facts hold:
\begin{enumerate}
\item[\textbf{Fact 1}] $|\psi_p(f) - \psi_p(f_0)|\leq ||\deriv{x_p}f - \deriv{x_p}f_0||_n^2$
\item[\textbf{Fact 2}]  
$\sup_{p \in \{1, \dots, P\}} ||\deriv{x_p}f - \deriv{x_p}f_0||^2_n \leq C * ||f - f_0||^2_n$ for some constant $C$.
\item[\textbf{Fact 3}]  
$\sup_{p \in \{1, \dots, P\}}|\psi_p(f_0) - \Psi_p(f_0)| \lesssim ||f - f_0||^2_n$. 
%This can be done using standard concentration inequality in Hilbert space (e.g. Lemma 18 of  \citep{rosasco_nonparametric_2013}), and is usually guanranteed since the rate is usually $n^{-\frac{1}{2}}$. Also notice that it is a constant with respect to the posterior distribution.
\end{enumerate} 
Because if above facts hold, we then have
\begin{align*}
\sup_{p\in \{1, \dots, P\}}|\psi_p(f) - \Psi_p(f_0)| &\leq 
\sup_{p\in \{1, \dots, P\}}|\psi_p(f) - \psi_p(f_0)| + \sup_{p\in \{1, \dots, P\}}|\psi_p(f_0) - \Psi_p(f_0)| \\
&\leq \sup_{p\in \{1, \dots, P\}}||\deriv{x_p}f - \deriv{x_p}f_0||^2_n + \sup_{p\in \{1, \dots, P\}}|\psi_p(f_0) - \Psi_p(f_0)|\\
& \leq C * ||f - f_0||^2_n + 
\sup_{p\in \{1, \dots, P\}}|\psi_p(f_0) - \Psi_p(f_0)|\\
& \lesssim ||f - f_0||^2_n,
\end{align*}
it then follows that:
\begin{align*}
E_0\Pi_n \Big(\sup_{p\in \{1, \dots, P\}}|\psi_p(f) - \Psi_p(f_0)| \geq M_n \epsilon_n \Big) 
& \lesssim
E_0\Pi_n \Big( ||f - f_0||^2_n \geq M'_n \epsilon_n \Big)
\rightarrow 0.
\end{align*}

We now show Facts 1-3 are true: 
\begin{itemize}
\item \textbf{Fact 1} follows simply from the triangular inequality:
\begin{align*}
|\psi_p(f) - \psi_p(f_0)| 
&= 
\Big| ||\deriv{x_p} f ||_n^2 - ||\deriv{x_p} f_0 ||_n^2 \Big|\\
&= 
\max\Big\{
||\deriv{x_p} f ||_n^2 - ||\deriv{x_p} f_0 ||_n^2,\;
||\deriv{x_p} f_0 ||_n^2 - ||\deriv{x_p} f ||_n^2
\Big\}
\leq ||\deriv{x_p} f_0 - \deriv{x_p} f ||_n^2.
\end{align*}
\item \textbf{Fact 2}. First establish some notation. Given data $\{\bx_i, y_i\}_{i=1}^n$, denote $\bdf$ and $\bdf_0$ the $n \times 1$ vectors with their elements being $f(\bx_i)$, $f_0(\bx_i)$, respectively. We then have 
$||f - f_0||^2_n = ||\bdf - \bdf_0||^2_2$. Furthermore, 
since $f, f_0 \in \Fsc(L, W, S, B)$, there exisits sets of weight matrices $\{\bW_l, \bS_l\}_{l=1}^L$, $\{\bW_{0,l}, \bS_{0,l}\}_{l=1}^L$ and output weights $\bbeta, \bbeta_0$ such that $
\bdf = \bX\bW_1\bS_1 (\prod_{l=2}^L \bW_l\bS_l)\bbeta$ and $\bdf_0 = \bX\bW_{0,1}\bS_{0,1} (\prod_{l=2}^L \bW_{0,l}\bS_{0,l})\bbeta_0$. To keep the notation simple, we write for $\bdf$ its the input weights as $\bW$, and the product of weight matrices after the input layer as $\bD = \bS_1 (\prod_{l=2}^L \bW_l\bS_l)\bbeta$, such that $\bdf$ and $\bdf_0$ can be written as:
\begin{align*}
\bdf &= \bX\bW\bD, \quad 
\bdf_{0} = \bX\bW_{0}\bD_{0}
\end{align*}
where recall $\bX$ is a $n \times nP$ block diagonal matrix with $1 \times p$ vectors $\bx_{i}$'s on the diagonal. Furthermore, by the definition of gradient functions for  \gls{ReLU} network, we can write the $n \times 1$ vectors of gradient functions as: 
\begin{align*}
\partial_p \bdf = \bW_p\bD, \quad 
\partial_p \bdf_0 = \bW_{0,p}\bD_0,
\end{align*}
where $\bW_p = \bI_n \otimes \bw_p, \bW_{0,p} = \bI_n \otimes \bw_{0,p}$ are $n \times nK$ block diagonal matrices. Notice that $||\deriv{x_p}f - \deriv{x_p}f_0||^2_n = ||\partial_p \bdf - \partial_p \bdf_0||^2_2$.
Finally, we will denote $\bbX = [\bX^\top, \dots, \bX^\top]^\top$ a $nP \times nP$ matrix that is formed by stacking $\bX$ for $P$ times.

Consequently:
\begin{align*}
\sup_{p \in \{1, \dots, P\}} ||\deriv{x_p}f - \deriv{x_p}f_0||^2_n 
&\leq \sum_{p=1}^P ||\deriv{x_p}f - \deriv{x_p}f_0||^2_n \\
&= \sum_{p=1}^P ||\bW_p\bD - \bW_{0,p}\bD_{0}||^2_2 
= ||\bW\bD - \bW_0\bD_{0}||^2_2 
\\
&\leq ||\bbX^{-1}\bbX(\bW\bD - \bW_0\bD_{0})||^2_2 
\leq ||\bbX^{-1}||_2^2||\bbX\bW\bD - \bbX\bW_0\bD_{0}||^2_2\\
&= P * ||\bbX^{-1}||_2^2||\bX\bW\bD - \bX\bW_0\bD_{0}||^2_2
= P * ||\bbX^{-1}||_2^2||f - f_0||^2_n \\
&\leq \frac{P}{c_x} ||f - f_0||^2_n.
\end{align*}
The equality on the fourth line follows since $||\bbX(\bW\bD - \bW_0\bD_{0})||^2_2 = P * ||\bX(\bW\bD - \bW_0\bD_{0})||^2_2$, due to the fact that $\bbX$ is formed by stacking the $\bX$ matrix $P$ times. We can assume without loss of generality that for $\bx_i = \{x_{i,p}\}_{p=1}^P$, $x_{i, p}$ is always bounded away from zero by a small constant $c_x > 0$, such that $x_{i, p} \geq c_x \forall i, p$.
Then the inequality on the last line follows since $||\bbX^{-1}||_2$ is bounded by $\frac{1}{c_x}$. This is because $||\bbX^{-1}||_2 = \lambda_{max}(\bbX^{-1}) = 1/\lambda_{min}(\bbX)$, and $\bbX$ can be re-ordered (through column permutation) into a block matrix with $P \times P$ diagonal matrices $\bX_i = diag(x_{i,1}, \dots, x_{i,p})$, such that:
$\bbX = \begin{bmatrix}
\bX_1 & \bX_2 & \dots & \bX_n\\
\bX_1 & \bX_2 & \dots & \bX_n\\
\dots & \dots & \dots &  \dots\\
\bX_1 & \bX_2 & \dots & \bX_n\\
\end{bmatrix}$.
Since eigenvalues of $\bbX$ is invariant under column permutation, and eigenvalue of a block matrix is the eigenvalues of the matrix blocks on the diagonal, we see that $\lambda_{min}(\bbX) = min_{i,p}(x_{i,p}) \geq c_x$. Consequently, since $\frac{P}{c_x} = O_p(1)$, we have shown that for some constant $C$:
\begin{align*}
\sup_{p \in \{1, \dots, P\}} ||\deriv{x_p}f - \deriv{x_p}f_0||^2_n \leq C * ||f - f_0||^2_n
\end{align*}
\item \textbf{Fact 3} follows from standard Bernstein-type concentration inequality (see, e.g. Lemma 18 of \cite{rosasco_nonparametric_2013}). Specifically, for $|\deriv{x_p}f_0(\bx)|^2$ a random variable with respect to probability measure $P(\bx)$ that is bounded by $L$. Given $n$ \gls{iid} samples $\{|\deriv{x_p}f_0(x_i)|^2\}_{i=1}^n$, recall that $\hat{\psi}(f_0) = \frac{1}{n}\sum_{i=1}^n |\deriv{x_p}f_0(x_i)|^2$ and $\psi(f_0) = E(\deriv{x_p}f_0)$, then with probability $1 - \eta$:
\begin{align*}
|\hat{\psi}(f_0) - \psi(f_0)| \leq 
n^{-\frac{1}{2}} * \big(2\sqrt{2} * L * log(2/\eta)\big),
\end{align*}
that is, $|\hat{\psi}(f_0) - \psi(f_0)| \rightarrow 0$ at rate of $O(n^{-\frac{1}{2}})$. Notice that $O(n^{-\frac{1}{2}})$ is the optimal parametric rate that cannot be surpassed by the convergence speed of the \gls{ReLU} networks (recall the typical convergence rate is $\epsilon_n \asymp n^{-\frac{\beta}{2\beta + \delta}}*log(n)^\gamma$ for some $\delta > 0$ and $\gamma > 1$). Therefore we have:
$$
\sup_{p \in \{1, \dots, P\}}|\psi_p(f_0) - \Psi_p(f_0)| \lesssim ||f - f_0||^2_n.
$$
\end{itemize}


==> sections/proof/sparsistency.tex <==
Show the statement by showing that $\hat{A}_n \supset A_0$ and $\hat{A}_n \subset A_0$ under $\Pi_n$ for sufficiently large $n$.

First show $\hat{A}_n \subset A_0$, i.e. $\hat{A}_n$ asymptotically prunes out all the irrelevant variables. Show this by contradiction, i.e. assuming $\exists p$ a variable index such that $p \in \hat{A}_n$ and $p \not\in A_0$. Notice that for the $(1-\alpha)$-level credible interval $\hat{B}_n=\{\hat{B}_{n,p}\}$ (i.e., $\Pi_n(\hat{\psi}^c_p(f) \in \hat{B}_n) = 1-\alpha$), $p \in \hat{A}_n$ implies that $0 \not\in \hat{B}_n$, i.e. $\psi^c_p(f)=\psi_p(f)-\eta_n$ is bounded away from zero. 

Therefore, for $n \rightarrow \infty$ and $\epsilon_n$ the given rate of convergence of the \gls{ReLU} network, there always exists a sequence $M'_n>0$ such that:
\begin{align}
E_0\Pi_n \Big(|\psi_p(f) - \Psi_p(f_0)| > M_n \epsilon_n\Big) 
&=
E_0\Pi_n \Big(|\psi_p(f)| > M_n \epsilon_n\Big) 
\nonumber\\
&\geq E_0\Pi_n \Big(|\psi^c_p(f)| - |\eta_n| > M_n \epsilon_n\Big) 
\nonumber
\\
&\geq E_0\Pi_n \Big(|\psi^c_p(f)| > M'_n \epsilon_n\Big)
\\
& \geq E_0\Pi_n (\hat{B}_{n,p}) \geq E_0\Pi_n (\hat{B}_n) 
= 1-\alpha > 0, \label{eq:subset_contradict}
\end{align}
where the first line follows since $p \not\in A_0$ implies $\Psi_p(f_0)=0$, the second line follows by triangular inequality and the definition of $\psi^c_p(f)$, the third line follows since $\eta_n \lesssim \epsilon_n$ due to the fact that $\eta_n=E(\inner{H_p\omega}{\omega})=O(tr(H_p)/n)=O(K/n) = o_p(n^{-\frac{1}{2}}) \lesssim \epsilon_n$, therefore we can always find a large enough $M'_n$ such that $M'_n\epsilon_n > M_n\epsilon_n + |E(\eta_n)|$. On the last line, the first inequality follows from the fact that $0 \not\in \hat{B}_{n,p}$ implies $|\psi_p(f)|$ is bounded away from zero, and the second inequality follows since for a simutaneous confidence interval $\hat{B}_n =\{\hat{B}_{n,p}\}_{p=1}^P$, the coverage probability of the marginal interval $\hat{B}_{n,p}$ is always greater than that of the joint interval $\hat{B}_n$. 

However, (\ref{eq:subset_contradict}) essentially implies that the posterior distribution $\psi_p(f)$ does not converge toward $\Psi_p(f_0)$, which contradicts with Theorem \ref{thm:post_convergence}, we therefore conclude that $\hat{A}_n \subset A_0$.\\

Now show $\hat{A}_n \supset A_0$, i.e. $\hat{A}_n$ asympotically retains all the truely informative variables. Assume not, i.e. $\exists p$ such that $p \in A_0$ but $p \not\in \hat{A}_n$. This implies that $\Psi_p(f_0) > 0$ while $0 \in \hat{B}_{n,p}$.

We will show contradiction by showing $\Psi_p(f_0)$ in fact converge to $0$ under the posterior distribution. For any sequence $M_n \rightarrow \infty$, we have
\begin{align*}
E_0\Pi_n(|\Psi_p(f_0)| \geq M_n \epsilon_n) 
& \leq 
E_0\Pi_n\Big(
|\Psi_p(f_0) - \psi_p(f)|+|\psi_p(f)|\geq M_n \epsilon_n \Big)\\
&\leq
E_0\Pi_n\Big(
\big\{|\Psi_p(f_0) - \psi_p(f)|\geq M_n \epsilon_n/2\big\} 
\cup 
\big\{|\psi_p(f)|\geq M_n \epsilon_n/2 \big\} \Big)
\\
& \leq 
E_0\Pi_n(|\Psi_p(f_0) - \psi_p(f)|\geq M_n \epsilon_n/2) + E_0\Pi_n(|\psi_p(f)|\geq M_n \epsilon_n/2)
\end{align*}
Notice the first term in the last line converges to 0 by Theorem \ref{thm:post_convergence}. So we only need to show $E_0\Pi_n(|\psi_p(f)|\geq M_n \epsilon_n/2) \rightarrow 0$. Because if this is true, then 
\begin{align*}
E_0\Pi_n(|\Psi_p(f_0)| \geq M_n \epsilon_n) \rightarrow 0,
\end{align*}
which implies that $\Psi_p(f_0)=0$, i.e. $p \not\in A_0$. This contradicts with the fact that $p \in A_0$. Therefore $\hat{A}_n \supset A_0$ and we have shown the statement of interest.

To show $E_0\Pi_n(|\psi_p(f)|\geq M_n \epsilon_n/2) \rightarrow 0$,  we notice that for any positive sequence $M_n \rightarrow \infty$:
\begin{align*}
E_0\Pi_n(|\psi_p(f)|\geq M_n \epsilon_n) 
&= 
E_0\Pi_n(|\psi^c_p(f) + \eta_n|\geq M_n \epsilon_n)\\
&\leq 
E_0\Pi_n(|\psi^c_p(f)| + |\eta_n|\geq M_n \epsilon_n)\\
&\leq 
E_0\Pi_n(
\big\{|\psi^c_p(f)|\geq M_n \epsilon_n/2 \big\} \cup 
\big\{|\eta_n|\geq M_n \epsilon_n/2 \big\})\\
&\leq 
E_0\Pi_n(|\psi^c_p(f)|\geq (M_n/2)* \epsilon_n) +  
E_0\Pi_n(|\eta_n|\geq (M_n/2)* \epsilon_n)\\
&\leq 
E_0\Pi_n(|\psi^c_p(f)|\geq M'_n* n^{-\frac{1}{2}}) +  
E_0\Pi_n(|\eta_n|\geq M'_n* \epsilon_n)
\end{align*}
where the last line follows since $\epsilon_n \gtrsim O(n^{-\frac{1}{2}})$, therefore we can always find another sequence $M'_n \rightarrow \infty$ such that $(M_n/2)* \epsilon_n \geq M'_n* n^{-\frac{1}{2}}$. Notice that both terms on the last line converge to 0 due to the fact that $\eta_n = o_p(n^{-\frac{1}{2}}) \leq \epsilon_n$ (as argued previously) and the fact that $|\psi^c_p(f)| = o_p(n^{-\frac{1}{2}})$. Specifically, $|\psi^c_p(f)| \lesssim O(n^{-\frac{1}{2}})$ follows from the fact that $0 \in \hat{B}_n$ and the fact that the width of confidence interval $\hat{B}_{n,p}$ shrinkage asymptotically at a rate of $n^{-\frac{1}{2}}$ (due to Theorem \ref{thm:bvm}), which implies $|\psi^c_p(f)|=|\psi^c_p(f)-0|<\mbox{width}(\hat{B}_{n,p})=O(n^{-\frac{1}{2}})$. Consequently, we conclude that
\begin{align*}
E_0\Pi_n(|\psi_p(f)|\geq M_n \epsilon_n)  \rightarrow 0.
\end{align*}


==> sections/related.tex <==
\subsection{Related Work}
\label{sec:lit_review}

This work encompasses three related areas of research: (1) model-based methods for nonlinear variable selection, (2) uncertainty quantification in variable selection, and (3) theoretical developement for Bayesian machine learning procedures. We review each of these three areas in the following subsections.

\subsubsection*{Nonlinear Variable Selection}

Most early modern works in variable selection focuses on the linear model, and a majority of them are developed under the a regularized-likelihood framework \citep{fan_selective_2010}. Classic examples include the non-negative garrote \citep{breiman_estimating_1985}, the \gls{LASSO}, \citep{tibshirani_regression_1996, yuan_model_2006}, elastic net \citep{zou_regularization_2005}, and the \gls{SCAD} \citep{fan_variable_2001}. 


The later works studying variable selection in nonlinear problems can be roughly grouped into three categories depending on the type of model being used: linear model, assumption-based nonlinear model (e.g., \gls{GAM}), and assumption-free nonlinear model (e.g., blackbox model such as kernel methods). The linear-model approaches perform variable selection by fitting a regularized linear model to the nonlinear data, and study the theoretic performance of variable selection under such model misspecification (see, e.g., \cite{zhang_consistency_2016}). The second approach (assumption-based nonlinear model) imposes explicit assumption on the functional dependency between the input variables and the outcome (i.e., additive effect, or interaction effect up to certain limited order). The modeling is commonly carried out under the \gls{GAM} framework and the variable selection is performed using (group) shrinkage estimators. Classic examples under this approach includes \cite{ravikumar_sparse_2007, meier_high-dimensional_2009, huang_variable_2010} for additive models, and \cite{lin_component_2006, bien_lasso_2013} for limited-order interaction models. The third approach completely removes the  assumptions on the structure of the data-generation function by fitting to the data assumption-free, blackbox models. Popular examples under this category includes the tree-based ensemble (e.g., \gls{RF} \citep{genuer_variable_2010} and \gls{BART} \citep{bleich_variable_2014}) that performs variable selection by thresholding each variables' inclusion probability to individual trees, and also kernel-method based approaches that assumes the data-generation function lies in certain pre-defined \gls{RKHS} \citep{wahba_advances_1999}. The kernel-based approaches measures the importance of a input variable using the squared norm of the gradient functions $\psi_p(f)=||\deriv{x_p}f||_n^2$, and perform variable selection through regularization \citep{ye_learning_2012, rosasco_nonparametric_2013, yang_model-free_2016} or thresholding \citep{he_scalable_2018}. By establishing the formal correspondence between the function space constructed by a deep neural network and a \gls{RKHS}, our definition of variable importance is consistent with this line of work.

Neural network is another popular model choice for assumption-free variable selection. A common approach under this category is to apply group-based shrinkage (e.g. group \gls{LASSO} or elastic net) to the input weights. Recent examples include \cite{feng_sparse_2017} for single-layer neural network and 
\cite{scardapane_group_2017} for deep neural networks. \cite{li_deep_2016} applied this approach to select DNA regulatory elements that impacts gene expression through complex pathways.
Moving beyond the regularization-based appraoch, some recent work has focused on extending other classic variable selection frameworks to the neural network model. For example, \cite{lu_deeppink:_2018} and \cite{romano_deep_2018} designed specialized network architecture to apply the knockoffs framework  \citep{barber_controlling_2015} to deep learing, and \cite{ye_variable_2018} designed a loss-based utility function to apply the idea of feature screening \citep{fan_nonparametric_2011, cui_model-free_2015} with neural networks. Finally, there also exist Bayesian approaches to variable selection based on shallow networks, focusing primarily on designing specialized,  sparse-inducing prior distribution on the input weights, and construct decision rule based on posterior point estimates (e.g., posterior mean). For example, \cite{beam_bayesian_2014} considered the \gls{ARD} prior on the variance of the input weights. \cite{liang_bayesian_2018} placed spike-and-slab prior with  identifiability constraints on the input weights and constructed decision rule by thresholding the inclusion probability for each input variable. In comparison, the algorithm proposed in this work performs variable selection using credible intervals. It does not require specially designed prior distribution or likelihood constraints, compatible with both shallow and deep architecture, and allows direct control over its precision-recall performance. 

\subsubsection*{Uncertainty Quantification in Variable Selection}

Under the frequentist paradigm, uncertainty quantification is a procedure that is separate from estimation, and usually involves constructing confidence interval or hypothesis testing procedures based on asymptotics theory for regularized estimators (i.e. the post-selection inference). There exisits several technical challenges to this approach, e.g. the non-continuity in the loss function and the biasedness in parameter estimates. \cite{lockhart_significance_2013, javanmard_confidence_2014, van_de_geer_asymptotically_2014, lee_exact_2016} are milestones in the theoretic developement along this direction. 

On the Bayesian side, uncertainty quantification for variable selection is commonly approached from the perspective of shrinkage priors. Notable work under this approach includes \cite{mitchell_bayesian_1988} , who introduced the spike and slab prior for specifically seeking a posterior probability of a model; stochastic search variable selection (SSVS) \citep{george_variable_1993, george_approaches_1997}; empirical Bayes variable selection \citep{george_calibration_2000}; spike-and-slab variable selection \citep{ishwaran_spike_2005}. See  \citep{ohara_review_2009} and \citep{clyde_model_2004} for a comprehensive review. Among the more recent developments, there are 
the non-local prior, \citep{johnson_bayesian_2012}; Bayesian shrinking and diffusing (BASAD) prior \citep{narisetty_bayesian_2014}; and Spike-and-Slab \gls{LASSO} \citep{rockova_spike-and-slab_2018}. Finally, we would like to note the work of \cite{bondell_consistent_2012} which uses the idea of penalized credible regions to perform variable selection under linear model. Our work generalized this idea to deep neural networks and provided theoretical justification to this approach through \gls{BvM} theorem.


\subsubsection*{Learning Theory for Bayesian Machine Learning Procedures}

Owning to the developement in modern Bayesian nonparametric theory, in recent years the literature has witnessed rapid advancement in the understanding the theoretical behavior of nonparametric, blackbox models  \citep{rousseau_frequentist_2016, ghosal_fundamentals_2017}. One major interest in the studies of the Bayesian learning procedures is their asymptotic frequentist properties. Given the posterior distribution of a model parameter, the common properties of interest include (1) \textit{posterior consistency} and  \textit{concentration rates}, i.e. whether and how fast the posterior distribution concentrates its probability mass around the true parameter as the sample size grow, and the (2) \textit{\glsfirst{BvM} theorem}, i.e. whether the asymptotic shape of the posterior distribution converge toward a Gaussian distribution. The first property informs the learning accuracy of the Bayesian procedure in finite sample, while the latter property provides frequentist justification for the practice of using posterior interval estimates to characterize a model's epistemic uncertainty. 

Among the popular blackbox methods, \glsfirst{GP} is one of the earliest to receive a thorough theoretical treatment. The general conditions for posterior convergence and the corresponding concentration rate are established in, for example, \cite{van_der_vaart_rates_2008, van_der_vaart_information_2011}. Results on the asymptotic normality in \gls{GP} arrives later, due to the well-known difficulty in establishing a \gls{BvM} theorem in the infinite-dimensional setting \citep{freedman_wald_1999}. Among these, we mention the semi-parametric \gls{BvM} result for finite-dimensional functionals by \cite{castillo_semiparametric_2012}, the nonparametric \gls{BvM} results for the full model posterior by  \cite{castillo_nonparametric_2013, castillo_bernsteinvon_2014}, and a dedicated investiagtion of simultaneous credible sets under the Gaussian process regression model by \cite{yang_frequentist_2017}. \glsfirst{BART} has also received considerable theoretic interest in the recent years. Leveraging its connection with the random histogram density model, \cite{rockova_posterior_2017} and \cite{rockova_theory_2018} established optimal rate of posterior convergence for various types of tree priors, and \cite{rockova_semi-parametric_2019} established an (adaptive) semi-parametric \gls{BvM} result for general smooth linear functionals.

There exists relatively few theoretical study on Bayesian neural networks. Among the known results, \cite{lee_consistency_2000} established the posterior consistency of one-layer Bayesian neural network for learning continous or square-integrable functions.  \cite{rockova_posterior_2018} generalized this result to deep architectures and to more general function spaces. They showed that, for the space of H\"{o}lder $\beta$-smooth functions, the rate of contraction almost attain the nonparametric minimax rate of $O(n^{-2\beta/(2\beta+d)})$. Finally, there does not seem to exist an \gls{BvM} results for the (deep) neural network models. Our work addresses this methodology gap by developing a semi-parametric \gls{BvM} theorem for a multivariate quadratic functional $\psi(f)=\{||\deriv{x_p}(f)||_n^2\}_{p=1}^P$.



==> sections/theory_learning.tex <==
\begin{comment}
To prepare notations for theoretical analysis, we define two operators $D_p$ and $H_p$:
\begin{align}
D_p(f)(\bx) = \inner{\deriv{x_p} k(\bx, .)}{f}_{\Hsc}, \quad 
H_p(f)(\bx) = \inner{\hat{h}_p(\bx, .)}{f}_{\Hsc}
\label{eq:operator_def}
\end{align}
such that $\psi_p(f)=||D_p(f)||^2_n = \inner{H_p(f)}{f}_{\Hsc}$. Furthermore, denote $\bK_\Wsc$ the $n \times n$ kernel matrix such that $(\bK_{\Wsc})_{i,j} = k_\Wsc(\bx_i, \bx_j)$, and $\bH_p$ the $n \times n$ gradient matrix such that $(\bH_p)_{i,j} = \hat{h}_p(\bx_i, \bx_j)$. Notice that $\bK_{\Wsc}$ and $\bH_p$ can be expressed simply in terms of the basis function matrices $\Phi$ and $\partial_p\Phi$:
\begin{align}
\bK_{\Wsc} &= \bPhi\bPhi^\top, \quad \bH_p = (\partial_p\Phi)(\partial_p\Phi)^\top
\label{eq:K_H_def}
\end{align}
where recall $\Phi_{n \times K}=\bX\bW_1\bS_1(\prod_{i=1}^L \bW_l\bS_l)$ and $(\partial_p\Phi)_{n \times K}=\bW_{1,p}\bS_1(\prod_{l=2}^L \bW_l\bS_l)$.
\end{comment}


For understanding a deep \gls{ReLU} networks' ability in learning and uncertainty quantification for the importance of input variables, two important questions need to be answered: (1) \textit{learning accuracy}. i.e., does a \gls{ReLU} networks' good performance in prediction (i.e. in learning $f_0$) translates to that in learning the variable importance? (2) \textit{uncertainty quantification}. i.e., does \gls{ReLU} network properly quantifies its uncertainty about variable importance, such that its $95\%$ credible interval for $\psi_p(f)$ indeed covers the ``true" variable importance $\psi_p(f_0)$ for $95\%$ of the time? 

In this section, we develop new Bayesian nonparametric results for the deep \gls{ReLU} network to answer both questions in the affirmative. For learning accuracy, we show that a \gls{ReLU} network learns the variable importance $\Psi_p(f_0)$ in a rate that  is at least as fast as its rate in learning $f_0$ (Theorem \ref{thm:post_convergence}). For uncertainty quantification, we establish a \textit{\glsfirst{BvM} theorem} to show that  the posterior distribution of $\psi(f)$ converge quickly (i.e. in the parametric $O(n^{-1/2})$ rate) toward a Gaussian distribution, and the $(1-\alpha)$-level credible interval of the posterior distribution covers the truth $(1-\alpha)\%$ of the time (Theorem \ref{thm:bvm} and \ref{thm:bvm_mvn}). The \gls{BvM} theorems establish a rigorous frequentist interpretation for a Bayesian \gls{ReLU} network's credible intervals, and are essential in ensuring the validity of the credible-interval-based variable selection methods in controlling its operating characteristics such as the \glsfirst{FDR}.
To the authors' knowledge, this is the first work to study \gls{BvM} phenomenon under the deep Bayesian neural network models.

Throughout the theoretical analysis, we make below two basic assumptions about the data and the model:
\begin{assumption}[True Function]
The true function $f_0$ has bounded norm $|| f_0 ||_\infty \leq C_f$
\label{eq:f_norm_bound}
\end{assumption}
Assumption \ref{eq:f_norm_bound} is fundamental in learning theory and ensures that the learning problem is well-defined. An unbounded $f_0$ essentially leads to infinite value in the loss function, rendering the risk minimization framework infeasible.

\begin{assumption}[Model Size] The width of the \gls{ReLU} network model $\Fsc(L, K, S, B)$ does not grow faster than $O(n^{1/2})$, i.e. $K = o_p(n^{1/2})$
\label{eq:tr_H_bound}
\end{assumption}
Assumption \ref{eq:tr_H_bound} puts an weak requirement on the growth rate of network capacity with respect to the sample size. It constraints the model's effective capacity (i.e., the rank of the network's kernel matrix $K$) to ensure the total stochasticity in the  neural network model is managable, such that the posterior estimate for $\psi_p(f)$ is stable and converges quickly toward the truth, which is a essential condition for the \gls{BvM} theorem to hold. Assumption \ref{eq:tr_H_bound} is satisfied by most of the popular neural network architectures in practice. For example, in the ImageNet challenge which contains $1.4 \times 10^7$ images, most of the successful architectures including AlexNet, VGGNet, ResNet-152 and Inception-v3 all have $K=O(10^3)$ nodes in the output layer \citep{russakovsky_imagenet_2015, krizhevsky_imagenet_2012, simonyan_very_2014, szegedy_rethinking_2015, he_deep_2016}. From the perspective of approximation theory, this choice is not restrictive either. For example, the choice $K = O(n^{\frac{d}{d + 2\beta}}*log(n)^{-2}) = o_p(n^{1/2})$ leads to an (near minimax) approximation rate $n^{-\frac{\beta}{2\beta + d}} * log(n)^{\frac{2\beta}{d}}$ (see, e.g., Theorem 5 of \cite{schmidt-hieber_nonparametric_2017}).


\subsubsection{Posterior Consistency and Concentration Rates}
\label{sec:thm_consistency}

Our first result concerns a Bayesian \gls{ReLU} network's ability in accurately learning the variable importance $\Psi(f_0)=||\deriv{x_p}(f_0)||^2_2$ in finite sample. It states that, for a \gls{ReLU} network that learns the true function $f_0$ in a rate $\epsilon_n$ (in the sense of Definition \ref{def:post_conv}), its posterior distribution for variable importance $\psi_p(f)$ converge consistently to a point mass on the truth $\Psi(f_0)$, and in a speed that is not slower than $\epsilon_n$. 


\begin{theorem}[Rate of Posterior Concentration for $\psi_p$]
For $f \in \Fsc(L, K, S, B)$, assuming the posterior distribution $\Pi_n(f)$ contracts around $f_0$ with rate $\epsilon_n$, then the posterior distribution for $\psi_p(f)=||\deriv{x_p}f||^2_n$ contracts toward $\Psi_p(f_0)=||\deriv{x_p}f||^2_2$ at a rate not slower than $\epsilon_n$, i.e., for any $M_n \rightarrow \infty$
\begin{align}
E_0\Pi \Big( \sup_{p \in \{1, \dots, P\}} |\psi_p(f) - \Psi_p(f_0)| > M_n \epsilon_n 
\big| \{y_i, \bx_i\}_{i=1}^n \Big) \rightarrow 0.
\label{eq:psi_post_converg}
\end{align}
\label{thm:post_convergence}
\end{theorem}
\begin{proof}
See Section \ref{sec:post_convergence_proof}.
\end{proof}
Theorem \ref{thm:post_convergence} confirms two important facts. The first fact is that, despite the non-identifiablity of the network's hidden weights $\Wsc$, a \gls{ReLU} network can reliably recover the variable importance of the true function $\Psi(f_0)$. The second is that a \gls{ReLU} network learns the variable importance  in a speed that is no slower than learning the prediction function $f_0$, i.e. good performance in prediction translates to good performance in learning variable importance. Given the empirical success of deep \gls{ReLU} networks in learning high-dimensional prediction functions, Theorem \ref{thm:post_convergence} suggests that \gls{ReLU} network is an effective tool for learning variable importance in high dimension.

The learning rate in Theorem \ref{thm:post_convergence} is only an upper bound. In fact, classic semi-parametric statistics theory suggests that the asymptotic convergence rate of $\psi_p(f)$ can be improved to the order of $O(n^{-1/2})$ (after certain suitable transformation) due to the good smoothness property of the \gls{ReLU} gradient functional $\psi_p(f)$ \citep{van_der_vaart_asymptotic_2000}. This is confirmed by the two \glsfirst{BvM} theorems (Theorem \ref{thm:bvm} and \ref{thm:bvm_mvn}) in the next section, which states  show that after proper re-centering, the posterior distribution of $\psi_p(f)$ converges in $O(n^{-1/2})$ rate toward a Gaussian distribution that is centered around the truth.



==> sections/theory_uq.tex <==
\subsubsection{Uncertainty Quantification}
\label{sec:thm_bvm}

In this section, we first establish a univariate semi-parametric \gls{BvM} theorem for $\psi_p(f)$ under the deep \gls{ReLU} network's posterior (Theorem \ref{thm:bvm}), and then extend it to the the multivariate case for $\psi(f)=\{ \psi_p(f) \}_{p=1}^P$  to handle the issue of multiple comparison (Theorem \ref{thm:bvm_mvn}). Both theorems show that, after proper re-centering, the posterior distributions of the variable importance parameters converge in $O(n^{-1/2})$ rate to a (multivariate) Gaussian distribution. More importantly,  this Gaussian distribution's credible intervals achieve the correct frequentist coverage for the true parameter.  

We first introduce the re-centering transformation that is that is necessary for the variable importance $\psi_p(f)$ to attain the \gls{BvM} phenomenon (i.e. asymptotic normality). Since the variable importance measure $\psi_p(f)=||\deriv{x_p}f||_n^2$ is non-negative, the \gls{BvM} phenomenon will not hold for $\psi_p$ when the true parameter lies on the boundary of the parameter space $[0, \infty)$, i.e., when $\psi_p(f_0)=0$. In this case, the $\Pi_n$ converges asymptotically to a Gamma distribution whose parameters changes depending on the specification of the prior  $\Pi(f, \Wsc)$ \citep{bochkina_bernsteinvon_2014}. For the purpose of constructing a variable selection rule, a Gamma asymptotic distribution is inconvinient since it does not center around the true parameter value $\psi(f_0)=0$, creating challenges for constructing decision rules using the posterior distribution. 

To avoid this complication, we consider a ``centered" version of $\psi_p(f)$:
\begin{align}
\psi^c_p(f) = \psi_p(f) - \eta_n,
\label{eq:psi_centered}
\end{align}
where $\eta_n$ is an bias correction term that estimates the  (asymptotically vanishing) bias between  $E\big(\psi_p(f)\big)$ and the true parameter $\psi_p(f_0)$ (see Theorem \ref{thm:bvm} for detail). We see that after centering, the parameter space of $\psi^c_p(f)$ now also includes negative values. As a result, the value of the true parameter $\psi_p(f_0)>0$ always lies in the interior of the parameter space, and the \gls{BvM} theorem wil always hold regardless of the value of the tru parameter:

\begin{theorem}[\glsfirst{BvM} for $\psi^c_p$]
For $f \in \Fsc(L, W, S, B)$, assuming the posterior distribution $\Pi_n(f)$ contracts around $f_0$ at rate $\epsilon_n$. Denote $D_p: f \rightarrow \deriv{x_p}f$ the differentiation operator, and $H_p = D_p^\top D_p$ the corresponding self-adjoint operator. For $\omega = Proj_\Fsc(\bepsilon)$, define:
\begin{alignat}{2}
\hat{\psi}_p &= ||D_p(f_0 + \omega)||_n^2
= 
\psi_p(f_0) + 2\inner{H_pf_0}{\omega}_n + \inner{H_p\omega}{\omega}_n, 
\label{eq:psi_estimator}
\end{alignat}
and its centered version as $\hat{\psi}^c_p=\hat{\psi}_p - \hat{\eta}_n$ where $\hat{\eta}_n=trace(H_p)$. 
Then $\hat{\psi}^c_p$ is an unbiased and efficient estimator of $\psi_p(f_0)$, and the posterior distribution for $\psi^c_p(f)$ is asymptotically normal surrounding $\hat{\psi}^c_p$, i.e.
\begin{align}
\Pi\Big(\sqrt{n}(\psi^c_p(f) - \hat{\psi}^c_p) 
\Big| \{\bx_i, y_i\}_{i=1}^n \Big) \leadsto N(0, 4|| H_pf_0 ||^2_n),
\label{eq:bvm}
\end{align}
\label{thm:bvm}
\end{theorem}
The proof is in Section \ref{sec:bvm_proof}. The proof utilizes the Bayesian \gls{ReLU} network's reprentation as a Gaussian process equipped with a \gls{ReLU}-network kernel function with hyperparameters $\Wsc$. The proof proceeds by first showing a \gls{BvM} phenomenon for a \gls{ReLU}-network Gaussian process with fixed $\Wsc$, and then show that \gls{BvM} still holds when $\Wsc$ is allowed to vary according to its posterior distribution $\Pi_n(\Wsc)$.

Theorem \ref{thm:bvm} establishes a rigorous theoretical basis for using the \gls{ReLU} network posterior $\Pi_n$ to quantify model uncertainty about variable importance. It states that the credible intervals from posterior distribution $\Pi_n\big(\psi^c_p(f)\big)$ achieves correct frequentist coverage (i.e. a $95\%$ credible interval covers the truth $95\%$ of the time). To see why this is the case, notice (\ref{eq:bvm}) implies that any random set $\hat{B}_n$ such that $\Pi_n\big(\psi^c_p(f) \in \hat{B}_n\big)=1-\alpha$ will satisfy:
\begin{align*}
\Pi_{N(0,1)}\big( (\hat{B}_n - \hat{\psi}^c_p)/\sigma_\psi \big) &\rightarrow 1 - \alpha
%\label{eq:bvm_ci_post}
\end{align*}
in probability for $\sigma_\psi^2=4|| H_pf_0 ||^2_n/n$, where we have denoted $\Pi_{N(0,1)}$ as the standard Gaussian measure. In other words, the set $\hat{B}_n$ can be written in the form of 
\begin{align}
\hat{B}_n = 
\Big[
\hat{\psi}^c_p - \rho_\alpha * \sigma_\psi, 
\hat{\psi}^c_p + \rho_\alpha * \sigma_\psi 
\Big],
\label{eq:bvm_ci}
\end{align}
i.e., it coincides with the $(1 - \alpha)$-level confidence intervals of an unbiased and efficient frequentist estimator of $\psi_p(f_0)$. As a result, similar to an efficient frequentist confidence interval, the credible interval (\ref{eq:bvm_ci}) achieves correct coverage for true parameter $\psi^c_p(f)$, and is optimal in the sense that its radius $\sigma_\psi$ attains the Cram\'{e}r-rao Lower Bound. As a result, $\hat{B}_n$ is the smallest possible interval that has the correct coverage \citep{kleijn_bernstein-von-mises_2012}.

Notice that Theorem \ref{thm:bvm} is an univariate result and provides justification only for the univariate confidence intervals. However, recall that performing variable selection in high dimension suffers from the issue of \textit{multiple comparison}, and decisions based only on univariate confidence intervals tend to have low precision and high \gls{FDR} (recall discussion in Section \ref{sec:intro}). Therefore we need to take the statistical dependencies between $\psi_p^c(f)$'s into account by considering the \textit{simutaneous credible interval} for the $P \times 1$ vector $\psi^c(f)=\{\hat{\psi}^c_p\}_{p=1}^P$.
To this end, we extending Theorem \ref{thm:bvm} to the multivariate case below to ensure the frequentist validity of a \gls{ReLU} network's simutaneous credible intervals.

\begin{theorem}[Multivariate \glsfirst{BvM} for $\psi^c$]
For $f \in \Fsc(L, W, S, B)$, assuming the posterior distribution $\Pi_n(f)$ contracts around $f_0$ at rate $\epsilon_n$.
For $\omega = Proj_\Fsc(\bepsilon)$, denote $\hat{\psi}^c=[\hat{\psi}^c_{1}, \dots, \hat{\psi}^c_P]$ for $\hat{\psi}^c_p$ as defined in Theorem \ref{thm:bvm}. Also recall that $P=O(1)$, i.e. the data dimension does not grow with sample size.

Then $\hat{\psi}^c$ is an unbiased and efficient estimator of $\psi(f_0)=[\psi_1(f_0), \dots, \psi_P(f_0)]$, and the posterior distribution for $\psi^c(f)$ asymptotically converge toward a multivariate normal distribution surrounding $\hat{\psi}^c$, i.e.
\begin{align}
\Pi\Big(\sqrt{n}(\psi^c(f) - \hat{\psi}^c) 
\Big| \{\bx_i, y_i\}_{i=1}^n \Big) \leadsto MVN(0, V_0),
\label{eq:mvn_bvm}
\end{align}
where $V_0$ is a $P \times P$ matrix such that $(V_0)_{p_1, p_2} =  4\inner{H_{p_1}f_0}{H_{p_2}f_0}_n$.
\label{thm:bvm_mvn}
\end{theorem}

\begin{proof}
See Section \ref{sec:mvn_bvm_proof}.
\end{proof}


